Sketch Then Generate: Providing Incremental User Feedback and Guiding LLM Code Generation through Language-Oriented Code Sketches

Crafting effective prompts for code generation or editing with Large Language Models (LLMs) is not an easy task. Particularly, the absence of immediate, stable feedback during prompt crafting hinders effective interaction, as users are left to mentally imagine possible outcomes until the code is generated. In response, we introduce Language-Oriented Code Sketching, an interactive approach that provides instant, incremental feedback in the form of code sketches (i.e., incomplete code outlines) during prompt crafting. This approach converts a prompt into a code sketch by leveraging the inherent linguistic structures within the prompt and applying classic natural language processing techniques. The sketch then serves as an intermediate placeholder that not only previews the intended code structure but also guides the LLM towards the desired code, thereby enhancing human-LLM interaction. We conclude by discussing the approach's applicability and future plans.

==> doc/3-code_ref.tex <==

\section{Text-Code Association in Prompts}
\label{sec:code_ref}

The goal of this work is to investigate the utilization of linguistic structures inherent in prompts for transforming them into code sketches. 
Central to this language-oriented approach is identifying the correspondences between the phrases and code elements. 
We refer a word or phrase within a prompt as a \emph{Code Reference}
if it specifically points to a piece of code (formally a node on the Abstract Syntax Tree~\cite{}).
These phrase-level references serve as anchor points, linking the prompt's linguistic structure to specific code elements, and play a crucial role to achieve our goal since we aim to update the code sketch incrementally as the user types.

% In analyzing how participants refer to code in their prompts, 
Specifically, we identify two types of code references: \emph{independent} and \emph{dependent}.

\begin{itemize}[leftmargin=*]
    \item \emph{Independent Reference} standalone points to code elements, typically employing the exact identifier of these elements (e.g., variable or function names) or reserved keywords. 
    The code referent of an independent reference can be precisely located without extra contextual information in the prompt. 
    For example, \zt{example} \textcolor{red}{(1) Converts $t_x$ and $t_y$ to pixel-based coordinates, (2) print the shape of $SalePrice$ in train.csv, (3) start reading data when you see \$ sign, stop reading data when you see \# sign, etc.}
    % when a participant uses "Initialize array dataStorage", "array" acts as an independent reference. The term directly points to a specific code construct, and dataStorage identifies the exact variable involved, allowing for clear and immediate identification within the codebase.
     \textcolor{red}{Edit code \textbf{above}; Add \textbf{this}, with model save name automated; the return type of \textbf{this} function is a node list }
     \textcolor{red}{\textbf{write} data to the serial port; \textbf{Convert} the string data to floating-point numbers}

    \item \emph{Dependent Reference}, on the other hand, refers to code elements through their relationship with other references within the prompt.
    The code referent of a dependent reference cannot be accurately located without additional information provided by the surrounding text.
    For example, \zt{example}
    % The referent of "it" (i.e., the array dataStorage) is understood only by considering its relationship with the independent reference that precedes it.
\end{itemize}

Identifying how a reference refer to code helps in developing strategies for parsing prompts as the user types and mapping them to code elements.
Next, we will describe how we develop our approach based on these code references.

% \subsubsection{Context of Code References: An Intermediate Level of Clarity}
% In our study, we found that users often refer to code elements when they possess an intermediate level of clarity about the desired code.
% Previous research~\cite{} has categorized user interactions with LLM-based programming assistants into two modes: acceleration, characterized by a clear vision of the intended code, and exploration, marked by uncertainty about the solution. 
% Our observations echo these distinctions, 
% revealing that users in exploration mode often 
% describe their problems rather than specify code elements, 
% utilizing tools like ChatGPT or Copilot Chat for guidance. 
% Conversely, those in acceleration mode lean towards direct code manipulation, 
% favoring features like Copilot's auto-completion instead of NL prompts.

% In addition to exploration and acceleration mode,
% we also noticed that participants often have an intermediate clarity of the intended code -- a state where the user possesses an overall conceptions of the necessary functions, variables, or code structures but lacks confidence in the finer details.  
% For instance, a user might request the creation of a \emph{``REST API with a GET handler to read from a database''}, 
% implying a clear idea of the desired code element (i.e., \emph{a GET handler}) 
% reveals ambiguity about how to achieve this functionality (i.e., how to \emph{read from a database}).
% This intermediary position encourages more frequent referencing of code elements as users seek to align the generated code with their project's architectural goals and details.
% In this intermediate clarity zone, 
% participants find Copilot Inline Chat or inline comments to be more suitable.

% It's crucial to acknowledge that our classification of user behavior represents a spectrum rather than discrete categories. Users dynamically transition among these states throughout the coding process, reflecting the fluid and dynamic nature of software development.
% These observations not only highlight the versatility required of LLM-based programming assistants 
% but also pinpoint the specific scenario where our Language-Oriented Code Sketching approach can offer the most value.


==> doc/_deprecated/1-intro_v0.tex <==
\section{Introduction }

With the advancement of Large Language Models (LLMs), the use of natural language (NL) prompts to generate or edit code has gained popularity in the programming domain~\cite{}. 
This transformative approach, while groundbreaking, introduces a spectrum of usability challenges. 
Programmers often navigate through
the intricacies of writing effective prompts~\cite{}
and understanding the LLM-generated code~\cite{}. 
These challenges are exacerbated by the ``black box'' nature of LLMs,
which forces users into iterative cycles of guesswork and adjustment~\cite{}.

Many existing methods have explored enhancing human-LLMs interactions in coding
by helping users write more effective prompts~\cite{}.
% or better interpret LLM-generated code suggestions~\cite{}.
Despite the value of these methods, they confront a fundamental problem: 
the slow feedback loop.
The delay between writing a prompt, submitting it, awaiting the generated code, and then evaluating the code undermines productivity and escalates frustration. 
This latency is a direct consequence of the computational demands of LLMs coupled with the iterative refinement process.

Imagine a paradigm shift towards \emph{``Live Prompting''} — a notion inspired by ``Live Programming''~\cite{}.
In this envisioned scenario, 
\emph{immediate, incremental feedback} is given with each modification of the prompt, potentially including generated code or other valuable intermediate results.
This feedback mechanism facilitate a smoother transition from prompt to  code, reducing the trial-and-error cycle. 
However, achieving Live Prompting presents significant challenges.
Continuously evaluating the user's prompt using LLMs as they type may not be a feasible solution, at least currently, due to the computational intensity and inherent unpredictability of LLM outputs. 
These constraints necessitate innovative approaches to realize the notion of Live Prompting beyond solely LLM reliance.

One observation, however, is that users' prompts frequently include phrases that directly reference code elements, embedded within narratives that mirror the structural relationships of the desired generated code.
Such a pattern points to a linguistic blueprint of the desired output, 
offering an interesting opportunity to approximate Live Prompting without reliance on LLMs. 
By mapping these phrases (such as \colorbox{mypink}{\texttt{Pytorch dataset}} and \colorbox{mypink}{\texttt{function}} in \autoref{fig:teaser}a) to predefined code snippets and then dynamically assembling them based on their linguistic context, 
we can transform prompts into code sketches using classic natural language processing techniques~\cite{}.
These sketches (\autoref{fig:teaser}b) not only provide immediate feedback to users 
but also serve as a foundational layer for LLMs to further refine and complete (\autoref{fig:teaser}c), offering a glimpse into a practical form of Live Prompting. 

This work thus explores how these linguistic cues could be used to enable language-oriented code sketching.
We focus on the scenarios where users \emph{use natural language prompts to generate or edit codes through LLMs}.
% offering a practical and efficient means to achieve a variant of live prompting.
We first analyze conducted a formative study to understand the prompts.
We propose an approach that convert prompts to code sketch instantly and incrementally, offering a feedback for the users when they are typing.
Further, the code sketches can server as a base to guide LLMs in generating codes,


Contribution:
- an approach, \method{}, that convert prompts to code sketch instantly and incrementally.
- a technique prob that implements the \method{}, as well as a set of novel interactive features to facilitate human-AI collaborations in programming.
- an evaluation xxx


%% LLM for coding is good, what it is? NLP --> Code

%% despite the good, it sucks. it sucks in multiple way, feedback is slow and huge, lacking of controllability.

%% Option2: To tackle these issues, we aim to provide instant, incremental feedback when the user is typing prompt.
%% we achieve this by leveraging the embedded structure in the prompt.

%% we propose a xx method. how applicable of our method.

%% our method is awesome.
%% Additionally, enable a set of new interactions and UX.

%% through a user study, xxx good



%%%%%%%%%

%% Option1: we atrribute these issues to Z. 
%% our key insight / observation is that there is rich sctructual information in the prompt that can be naturally used to create a code template/preview to provide an instant, incremental feedback for the user.

% The application and research of Large Language Models (LLMs) in coding have gained substantial traction, leading to their integration into a plethora of coding environments such as GitHub Copilot\footnote{https://github.com/features/copilot}, Tabnine\footnote{https://www.tabnine.com/}, and CodeWhisperer\footnote{https://aws.amazon.com/cn/codewhisperer/}, among others. 
% These advancements have markedly influenced coding methodologies and underscored the creative potential of LLMs within this domain. 
% Notably, LLMs have been employed in diverse contexts including code snippet generation~\cite{wermelinger2023using, bird2022taking}, 
% collaborative pair programming~\cite{dakhel2023github, imai2022github}, 
% the generation of technical documentation~\cite{liu2021haconvgnn}, 
% as well as in roles supportive of learning and mentorship~\cite{puryear2022github, becker2023programming, kazemitabaar2023novices}. 
% The core principle underlying LLMs in coding is the translation from natural language to code (NL2Code), which, despite its foundational role, reveals that LLMs' efficacy can fluctuate across different tasks and applications~\cite{chen2021evaluating}. 
% Moreover, the inherently stochastic nature of LLMs introduces challenges in terms of response latency and control, particularly when managing extensive contexts and feedback~\cite{kamradt2023needle}. 
% In light of these challenges, our research involves a contextual inquiry as a formative study wherein we observe programmers' interactions with LLMs in naturalistic settings. 
% This formative study, involving 11 participants, seeks to identify prevalent issues encountered when coding with LLMs, with the ultimate goal of developing a system that delivers immediate and incremental feedback during the user's engagement with the coding prompt.

% \textcolor{red}{We propose xxx method --> our method is awesome --> user study finding}



==> doc/_deprecated/1-intro_v2.tex <==
\section{Introduction}

The advent of Large Language Models (LLMs) represents a paradigm shift in programming, 
enabling an era where natural language (NL) prompts can directly inform code generation and editing~\cite{}. 
This advancement, while groundbreaking, 
% introduces a spectrum of usability challenges~\cite{}, 
% particularly in 
% Particularly, 
programmers often face the challenge of writing effective prompts 
% with appropriate level of detail and context 
to allow LLMs to generate the desired code~\cite{}.
Consequently, users often find themselves in a tedious loop of trial and error, 
continuously refining their prompts to reach their desired outcomes~\cite{}.

To address this gap, several methods have been developed,
such as Grounded Abstraction Matching~\cite{}, 
which translates code back into an example NL expression for further iteration, 
and the decomposition of complex prompts into more detailed sub-prompts~\cite{}. 
While these approaches have demonstrated their usefulness, 
they share a common issue:
the absence of immediate, stable feedback into the potential outcomes while crafting prompts.
This lack of such feedback can lead to uncertainty about the expected output, 
decreased user engagement, 
and potential inefficiencies in the development process, 
as users are left to mentally project possible outcomes until the code is generated~\cite{}.

Imagine a paradigm where, as soon as you type your prompt, 
a code sketch begins forming on your screen. 
This sketch, emerging instantly and evolving incrementally, 
is not the final generated code, but serves as an intermediate, meaningful placeholder
that offers a preview of the intended code structure of your prompt. 
Furthermore, 
the sketch enriches your prompt with details, 
guiding the LLM to generate the code you desire, 
akin to the ``sketch'' in programming synthesis~\cite{}.
This approach, which we term \emph{``Language-oriented Code Sketching''},
while not accelerating the underlying model computations, 
can facilitate the interaction between programmers and LLMs. 

However, realizing this approach presents significant challenges.
Continuously evaluating the user's prompt with LLMs to obtain the sketch may be currently impractical due to computational demands and the unpredictable nature of LLM outputs. 
These limitations call for innovative solutions beyond solely reliance on LLMs to achieve Language-Oriented Code Sketching.

One observation, however, is that users' prompts frequently include phrases directly referencing code elements, embedded within narratives that reflect the relationships among these elements in the intended code structure.
Consider the prompt \emph{``Define a Pytorch dataset with a loadImg function''} (\autoref{fig:teaser}a).
Here, \colorbox{mypink}{\texttt{Pytorch dataset}} and \colorbox{mypink}{\texttt{loadImg function}} reference a class and a function, respectively.
Their linguistic relationship -- where \colorbox{mypink}{\texttt{loadImg function}} is an object of the preposition \emph{``with''} modifying \colorbox{mypink}{\texttt{Pytorch dataset}} -- reveals that the function is meant to be a component of the class.
While the specific details of the code remain undefined,
this linguistic structure of the prompt offers an interesting opportunity to create code sketches without reliance on LLMs: 
by mapping these phrases to predefined code snippets and then assembling them based on their linguistic relationship,
we can transform a prompt into a code sketch (\autoref{fig:teaser}b) using classic natural language processing (NLP) techniques~\cite{}.
This sketch not only provide immediate feedback to users 
but also serve as a foundational layer for LLMs to further refine and complete (\autoref{fig:teaser}c), 
offering a practical form of Language-Oriented Code Sketching. 

This work thus explores how these linguistic structures could be used to enable Language-Oriented Code Sketching.
We focus on the scenarios where users use natural language prompts to generate or edit codes through LLMs.
We first conducted a formative study to understand why, how, and when users reference code in their prompts.
The finding reveals that \zt{xxxx}.
Informed by the study,
we design \method{}, an interactive approach that converts a prompt to a code sketch as the user is typing.
Through a user interface of auto-completion,
this method converts a prompt to a code sketch instantly and incrementally
without taxing users extra cognitive loads, also allowing users to interactively solving the ambiguities of the natural language.
We implement \method{} in a proof-of-concept system, with a set of novel interactive features, and report a comparative study
on the use of the system as a technology probe~\cite{}
to understand how Language-Oriented Code Sketching
facilitate human-AI coding.
The result shows that \zt{xxxx}.

Contribution:
\begin{itemize}
    \item an approach, \method{}, that convert prompts to code sketch instantly and incrementally.
    \item a proof-of-concept system as a technology probe that implements the \method{}, as well as a set of novel interactive features to facilitate human-AI collaborations in programming.
    \item an evaluation xxx
\end{itemize}

% Such a sketch not only aids further refinement but also enhances the interaction between the programmer and LLM by 
% providing a tangible blueprint that evolves in real-time with the user's input.
% The key philosopy, is that before building the big thing, we incrementally move small steps, and intemediate results.
% \emph{immediate, incremental feedback} is given with each modification of the prompt, potentially including generated code or other valuable intermediate results.



% Many existing methods attempt to bridge the abstraction gap by 
% helping users write more effective prompts~\cite{}.
% For example, Liu et al. introduced the
% technique of grounded abstraction matching, 
% which involves translating the code back into a NL expression which can be edited and used for futher iterations.
% Another major approach is to decompose complex prompts into sub-prompts
% of a pre-defined abstraction level~\cite{}. Specifically,
% the programming task is divided into smaller, more manageable
% sub-tasks, each at a set level of complexity or detail.
% Despite the value of these methods, 
% these solutions still rely heavily on LLMs to provide feedback. 
% still, they all require users to directly interact with LLMs, and need to wait for a long time to see the generated code as feedback.

% While there have been efforts within the domain to mitigate these challenges—ranging from techniques aimed at refining user prompts to strategies for decomposing complex tasks into simpler sub-prompts—these solutions still rely heavily on LLMs to provide feedback. 
% Such reliance not only sustains the feedback delay but also underscores the limitations of existing methodologies in offering a swift, interactive coding experience. 
% Moreover, though incremental code generation using LLMs has been explored, 
% the fundamental bottleneck of slow feedback remains unaddressed, 
% given the computational intensity and unpredictability of LLM outputs.



% This methodology, which we term \emph{Incremental Code Sketching (ICS)}, serves as a bridge between the user's conceptual intent and the LLM's powerful code generation capabilities. 
% By providing users with an immediate sketch of their code, we facilitate a dynamic dialogue between the programmer and the LLM. 
% This not only streamlines the coding process but also mitigates the cognitive load on the user, making the interaction with LLMs more intuitive and productive. 
% Through ICS, we leverage the strengths of LLMs for detailed, sophisticated code generation while addressing their limitations in speed and interactivity, presenting a balanced approach to modern coding challenges.

% ICS acts as a conduit between the user's conceptual intent and the LLM's robust code generation capabilities, fostering a dynamic exchange that reduces cognitive load and enhances productivity. By offering an immediate representation of the user's idea, ICS leverages LLMs' strengths in generating detailed code while addressing their limitations in responsiveness and user interaction, thus offering a nuanced solution to contemporary programming challenges.

% Imagine a paradigm shift towards \emph{``Live Prompting''} — a notion inspired by ``Live Programming''~\cite{}.
% In this envisioned scenario, 
% \emph{immediate, incremental feedback} is given with each modification of the prompt, potentially including generated code or other valuable intermediate results.
% This feedback mechanism facilitate a smoother transition from prompt to  code, reducing the trial-and-error cycle. 
% However, achieving Live Prompting presents significant challenges.
% Continuously evaluating the user's prompt using LLMs as they type may not be a feasible solution, at least currently, due to the computational intensity and inherent unpredictability of LLM outputs. 
% These constraints necessitate innovative approaches to realize the notion of Live Prompting beyond solely LLM reliance.

% they confront a fundamental problem: 
% the slow feedback loop.
% The delay between writing a prompt, submitting it, awaiting the generated code, and then evaluating the code undermines productivity and escalates frustration. 
% This latency is a direct consequence of the computational demands of LLMs coupled with the iterative refinement process.


%% LLM for coding is good, what it is? NLP --> Code

%% despite the good, it sucks. it sucks in multiple way, feedback is slow and huge, lacking of controllability.

%% Option2: To tackle these issues, we aim to provide instant, incremental feedback when the user is typing prompt.
%% we achieve this by leveraging the embedded structure in the prompt.

%% we propose a xx method. how applicable of our method.

%% our method is awesome.
%% Additionally, enable a set of new interactions and UX.

%% through a user study, xxx good




==> doc/_deprecated/2-related_v0.tex <==

\section{Related Work}

We reviewed relevant literature on the practices and challenges for coding with large language models (LLM), 
particularly for natural language to code, 
and structural code editors.

\subsection{Coding with LLM}
Recent advancements in LLMs have dramatically reshaped the landscape of software development. 
These AI-driven tools,
capable of generating syntactically correct and logically sound code from natural language prompts,
have unveiled a new frontier in programming efficiency and accessibility~\cite{}.
In essence, the advent of successful LLM-based coding tools (e.g., Github Copilot~\cite{}) has heralded a paradigm shift in how code is written.

The interaction between programmers and LLMs has been the subject of extensive research. 
Many studies~\cite{Kazemitabaar2023,nguyen2024beginning,prather2023} have delved into understanding the nuances of this interaction, 
focusing primarily on user behavior when using LLM-based coding assistants.
% Grounded copilot: How programmers interact with code-generating models, barke2023grounded
For instance, Barke et al.~\cite{barke2023grounded}
categorized the user behavior into acceleration mode, 
where the programmer has a clear conception of the code to be written, 
and exploration mode, 
where the programmer seeks guidance or inspiration due to uncertainty about the solution.
% Reading Between the Lines: Modeling User Behavior and Costs in AI-Assisted Programming
Mozannar et al.~\cite{} proposed CUPS, a taxonomy that characterizes the 
the programmers' activities when interacting with LLMs during coding tasks.
Notably, CUPS was developed based on data labeled by the participants themselves rather
than by the researchers interpreting their actions.
% An empirical Study of developer Behaviors for Validating and Repairing Ai-Generated Code
Tang et al.~\cite{} used eye-tracking data to analyze programmers' behaviors 
and found that they had a greater cognitive effort in editing AI-generated code.

Additionally, 
researchers have also identified serveral key usability issues when coding with AI assistants.
Crafting effective prompts is often challenging for users~\cite{sarkar2022like}, 
requiring a nuanced understanding of how LLMs interpret and respond to instructions,
also because enternalize the intention in natural langauge is challenging.
Verifying the accuracy and debugging of generated code can be difficult, particularly for users with limited programming expertise~\cite{vaithilingam2022expectation}. This can lead to an over-reliance on the tool, where users accept generated code without sufficient scrutiny.
The tools frequently lack controllability, 
leaving users with little influence over the nuances of input handling and output generation~\cite{Liang2023} and addressing the frequent misalignment between the models' outputs and the programmers' intentions~\cite{kou2023model}. 



While these studies offer invaluable insights into the interaction between programmers and LLMs, 
very few of them have reveal how the prompts look like.
Barke et al.~\cite{barke2023grounded} has brefily summarized that the prompt for guiding AI is different from the normal code comment. However, more details are missing.
In this study, we particularly are interested in 
understanding the programmer prompts in guiding LLMs within the context of 
their day-to-day development tasks outside the confines of a laboratory. 
% actual software development projects.

% A Large-Scale Survey on the Usability of AI Programming Assistants: Successes and Challenges

% What is it like to program with artificial intelligence? 
% Is Model Attention Aligned with Human Attention? An Empirical Study on Large Language Models for Code Generation, 

% predominantly focus on controlled, lab-based environments. 
% Such settings may not fully capture the complexities and variability of real-world coding projects. 
% The existing literature often overlooks the intricacies of how programmers craft prompts in 
% This gap in the research highlights a crucial area of inquiry: 

% Despite these advancements, the application of LLMs in coding presents notable challenges, particularly in understanding the underlying mechanisms of code generation by these models and 
% To Search or To Gen? Exploring the Synergy between Generative AI and Web Search in Programming, yen2024search
Moreover, it's common for programmers to adopt a hybrid approach, combining 'accelerate mode' and 'exploration mode', or combining generative AI and web search~\cite{yen2024search}, to optimize the coding process. 

Consequently, while LLMs like GitHub Copilot offer significant advantages in coding efficiency and exploratory learning, they also introduce complex challenges. 
These include the need for a deeper understanding of LLM-generated code, 
the alignment of code with programmers' intentions, 
and the risk of over-reliance, 
which may impair the development of fundamental programming skills and control over code structure. 
Addressing these challenges is crucial for maximizing the potential of LLMs in programming environments. 

The precise balance of the accelerate-exploration combination remains unclear, suggesting a need for further empirical studies to delineate the optimal integration of these modes. 
Understanding this balance is pivotal in refining the use of LLMs in coding, ensuring they serve as effective tools rather than crutches, 
thereby enhancing the programming landscape.


% Empirical research has extensively explored the integration of LLMs into programming practices, revealing their potential to enhance code generation efficiency~\cite{10.1145/3641289, % survey
% zan2023large, %survey
% sarkar2022like, 
% Nhan2022}. 
% GitHub Copilot stands out as a prominent example of LLM-based coding tools. 



\subsection{Natural Language Interface for Coding}

% "What It Wants Me To Say": Bridging the Abstraction Gap Between End-User Programmers and Code-Generating Large Language Models


%% what is Natural Language Interface (NLI)
%% it has been widely adopted in various domains
%% due to advance of LLM, it has now been used in programming -- copilot. In this work, we review NIL for coding.

%% text-to-code
%% bimodal (visual programming)
%% what's the difference or relationship with these prior work

%% Zeyu -- Version1:
% Leveraging the advancements in state-of-the-art models and algorithms for Natural Language to Code (NL2Code) conversion, researchers have developed a diverse range of interactive systems tailored for various coding applications. In the realm of end-user programming and code generation, efforts have been directed towards enabling code transformation and fostering programming approaches that are aligned with user intentions~\cite{liu2023wants, lahiri2022interactive, ni2021recode}. Additionally, there is a growing focus on creating exploratory and visual programming interfaces, which facilitate a more intuitive coding experience~\cite{edwards2004example, angert2023spellburst, cai2023low, huang2024anpl}. In the context of AI collaboration and assisted development, the research community has concentrated on two main areas: the development of collaborative interfaces and tools that enhance the synergy between programmers and AI~\cite{lee2022coauthor, ross2023programmer, feng2023coprompt}, and the integration of AI to streamline and enhance the programming workflow~\cite{mcnutt2023design, gebreegziabher2023patat, wu2022ai}. When it comes to UI/UX design and the visualization aspects of coding, there is significant work aimed at improving visual representations and the overall user experience in programming environments~\cite{asenov2016effect, vaithilingam2023towards, kim2022stylette}. This includes innovative approaches to code generation through visual abstraction techniques~\cite{yen2023coladder, arawjo2023chainforge, wu2022promptchainer}. Furthermore, the exploration of natural language interfaces for analytical purposes represents another vibrant area of research, underscoring the versatility and broad applicability of NL2Code technologies~\cite{setlur2016eviza, tian2023interactive}. This comprehensive body of work collectively contributes to the ongoing evolution of coding practices, making programming more accessible, efficient, and collaborative across a spectrum of applications.

% Despite advancements in interactive coding systems, challenges persist, including integrating user intentions with code transformation for end-user programming and developing intuitive, efficient user experiences for varied programming skills. Harmonizing programmer-AI collaboration, providing clear UI/UX visualizations, and balancing natural language flexibility with coding precision remain key hurdles. Overcoming these issues is crucial for the full potential of interactive programming systems.


%% Zeyu -- Version2:
Natural Language Interfaces (NLIs) are revolutionizing the way we interact with technology, enabling users to communicate with machines in their own language. 
This transformative approach has been widely adopted across various sectors, significantly enhancing user accessibility and interaction with complex systems. 
In the domain of programming, the advent of advanced Large Language Models (LLMs) has further propelled the use of NLIs, most notably through innovative applications like GitHub Copilot. This tool exemplifies the seamless translation of natural language into executable code, marking a significant milestone in the integration of human linguistic capabilities with computational processes. Building on this foundation, our work delves into the nuanced application of NLI within the coding landscape. We explore the diverse array of interactive systems developed through state-of-the-art models and algorithms for Natural Language to Code (NL2Code) conversion, tailored for a variety of coding applications. These systems range from end-user programming and code generation platforms designed to align with user intentions~\cite{liu2023wants, lahiri2022interactive, ni2021recode}, to exploratory and visual programming interfaces that offer a more intuitive coding experience~\cite{edwards2004example, angert2023spellburst, cai2023low, huang2024anpl}. Our review also covers the collaborative interfaces and AI integration efforts aimed at enhancing the synergy between programmers and AI technologies~\cite{lee2022coauthor, ross2023programmer, feng2023coprompt, mcnutt2023design, gebreegziabher2023patat, wu2022ai}, alongside the innovative approaches in UI/UX design for improved programming environments~\cite{asenov2016effect, vaithilingam2023towards, kim2022stylette, yen2023coladder, feng2023coprompt, arawjo2023chainforge, wu2022promptchainer}. This extensive body of work underscores the broad applicability and versatility of NL2Code technologies, pushing the boundaries of coding practices towards more accessible, efficient, and collaborative paradigms.

However, despite these advancements, challenges remain in fully realizing the potential of interactive coding systems. Key hurdles include integrating user intentions with accurate code transformation, developing intuitive interfaces for diverse programming skill sets, fostering effective programmer-AI collaboration, and achieving a balance between the flexibility of natural language and the precision required for coding. Addressing these challenges is imperative for advancing the field and unlocking the full capabilities of NLI-driven programming systems.

\subsection{Structural Code Editor}
%% directly edit the AST instead of chars
Structural code editors, which enable programmers to directly manipulate the high-level concepts (e.g. abstract syntax tree (AST)) rather than the textual code itself, represent a significant shift in the way code is edited and understood. This approach allows for a more intuitive interaction with the underlying structure of the code, ensuring that edits are syntactically correct by design. Building on this foundation, techniques such as those presented in~\cite{9127256} utilize toString functions to automatically generate graphical user interfaces (GUIs), making data structure manipulations within integrated development environments (IDEs) more accessible, particularly in programming by examples (PBE) or bidirectional transformations (BX) contexts. This fusion of direct code manipulation with user interaction is further exemplified in projects like~\cite{10.1145/3332165.3347925}, which blur the lines between making textual changes to the code and visually adjusting the graphical output, thereby offering a more integrated experience for creating SVG graphics. On the educational side, editors such as~\cite{10.1145/3397537.3397561} aim to make programming more approachable for beginners by ensuring that any code changes remain within the bounds of the language's syntax, thus smoothing the learning path. Similarly, GNOME~\cite{10.1145/800020.808250} leverages lessons from structural editing research to create an environment conducive to learning programming, especially for novices. The concerted efforts of these initiatives, along with a wide array of industrial projects~\cite{Lamdu91:online, Darklang73:online, TheUniso32:online, ensoorg70:online}, underscore the continuous innovation and diverse strategies within this domain, all aimed at reconciling the intuitiveness of graphical interfaces with the precision of textual programming.

However, while existing methods emphasize features like GUI generation, seamless graphical integration, and educational facilitation, they also highlight an area ripe for exploration: the language-oriented nature of structural code editors. This focus on tailoring editors to specific programming languages presents an opportunity to delve deeper into how these tools can adapt to diverse programming paradigms and environments. The challenge lies not in the language specificity itself but in expanding these editors' capabilities to accommodate a broader range of languages and development contexts. By exploring this area, the field can potentially address issues of adaptability and scalability, making structural code editors more universally applicable and enhancing their utility across various programming ecosystems.

\subsection{Natural Language to Code: Model \& Algorithms}

%% earlier stage: rule based, keyword-based snippet
%% preLLM: ML-based
%% LLM: werwer

% Zeyu -- Version 1
% To deepen our comprehension of the logic behind code generated by Large Language Models (LLMs), we explored existing literature on models and algorithms that facilitate the generation of code from natural language. At the very beginning, researchers proposed rule-based systems, for example,~\citet{winograd1980does} proposed SHRDLU, which could understand natural language commands within a block world.~\citet{feigenbaum1980knowledge} proposed the principles of expert systems and knowledge-based approaches in AI, which were also applicable to early NL2Code systems. Next, researchers proposed statistical methods and early machine learning~\cite{manning1999foundations, joachims1998text}. Next, work like GATE~\cite{cunningham2002gate} is proposed to figure out the keyword-based and pattern-matching techniques. Recently, a notable strategy involves organizing prompts into structured queries, which helps maintain the code's structural integrity~\cite{beurer2023prompting, elgohary2021nl}. Another approach is the transformation of prompts into a form of flow engineering, preserving structural patterns within the generated code~\cite{ridnik2024code, reynolds2021prompt}. Additionally, the implementation of Abstract Syntax Trees (AST) has been explored to parse generated code and establish connections with natural language constructs~\cite{yin2018tranx, 10.1145/3611643.3616323}. These methodologies underscore the relationship between grammar and semantics in code generation, aligning with deterministic rules and creative generation processes, respectively.

% Despite these advancements, the challenge remains in designing models that adeptly blend rule-based mechanisms with generative capabilities. In response to this challenge,~\citet{yin2017syntactic} introduced an innovative neural architecture that leverages a grammar model to incorporate the target grammar as prior knowledge, aiming to bridge the gap between rule-based precision and generative flexibility. This balance is crucial for enhancing the effectiveness and reliability of LLM-generated code.


% Zeyu -- Version 2
To enhance our understanding of the underlying principles guiding code creation by Large Language Models (LLMs), we delved into the scholarly works surrounding the models and algorithms enabling the translation of natural language into code. Initially, the field witnessed the introduction of rule-based systems, exemplified by~\citet{winograd1980does}, which demonstrated an ability to interpret natural language instructions within a simplistic block world environment. Building on these foundational concepts,~\citet{feigenbaum1980knowledge} laid the groundwork for expert systems and knowledge-based methodologies in artificial intelligence, principles that found early application in Natural Language to Code (NL2Code) systems. The subsequent phase of research shifted towards statistical methods and the nascent stages of machine learning, as illustrated by foundational works in the field~\cite{manning1999foundations, joachims1998text}.

Advancements continued with the introduction of frameworks like GATE, which refined the approach to identifying key phrases and patterns within text~\cite{cunningham2002gate}. In more recent developments, researchers have employed structured queries to enhance the structural coherence of the generated code~\cite{beurer2023prompting, elgohary2021nl}. Parallel to this, the concept of flow engineering has been employed to maintain the structural integrity within code generation~\cite{ridnik2024code, reynolds2021prompt}. The application of Abstract Syntax Trees (AST) represents another significant stride, facilitating the parsing of generated code and linking code structures with natural language elements~\cite{yin2018tranx, 10.1145/3611643.3616323}. These approaches collectively highlight the intricate interplay between grammatical rules and semantic understanding in code generation, marrying deterministic frameworks with the creative aspects of code production.

However, the integration of rule-based precision with the creative freedom of generative models remains a formidable challenge. Addressing this, Yin et al. introduced a groundbreaking neural framework that integrates a grammatical model to embed prior syntactic knowledge, aiming to harmonize the rigor of rule-based systems with the adaptability of generative models. This equilibrium is pivotal for bolstering the efficiency and dependability of code generated by LLMs~\cite{yin2017syntactic}.


==> doc/_deprecated/3-formative_study_v0.tex <==

\section{Formative Study}
\zt{WIP}
%% issue (1,2,3)
%% how to support our solution (4,5 abs level)

To better understand the real difficulties encountered by users when coding with LLM, we conducted a contextual inquiry (specifically focusing on GitHub Copilot) as a formative study, in which we observed in detail how users interact with LLM when they are not involved in an in-lab controlled coding task.

\subsection{Study Setup}
% - participants
% - procedure
% - analysis

\subsubsection{Participants}

We engaged 11 participants through a meticulous selection process, initiated by a screening questionnaire designed to gauge their programming proficiency and their familiarity and usage patterns with GitHub Copilot. The questionnaire comprised inquiries about their programming skill level on a 1 to 5 scale, the commencement and frequency of their GitHub Copilot usage, their proficiency with Copilot on a similar scale, and the primary types of projects for which they employ Copilot. Further questions delved into the challenges they faced while using Copilot, their most proficient programming languages, and the availability of a project they could demonstrate, including its programming language. This careful screening process was instrumental in assembling a diverse group of participants, each bringing unique insights into their experiences with GitHub Copilot, as summarized in Table~\ref{table: formative participants}.


\begin{table}[!tbh]
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
\hline
    & Programming Experience (Year) & Frequency of Coding with LLM & Coding Type                    \\ \hline
P1  & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P2  & 5+                            & Daily                        & Front-end Development          \\ \hline
P3  & 5+                            & Always                       & Front-end Development          \\ \hline
P4  & 5+                            & Always                       & Machine Learning                    \\ \hline
P5  & 5+                            & Monthly                      & Back-end Development           \\ \hline
P6  & 3-5                           & Daily                           & Back-end Development            \\ \hline
P7  & 3-5                           &  Always                       & Machine Learning                    \\ \hline
P8  & 5+                            &  Always                        &  Front-end Development        \\ \hline
P9  & 5+                              &  Daily                            &  Front-end Development      \\ \hline
P10 & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P11 & 1-2                              &  Weekly                            & Embedded Systems Development    \\ \hline
\end{tabular}
}


\caption{Participants in Formative Study}
\label{table: formative participants}
\end{table}

\subsubsection{Procedure}

Our study procedure is meticulously designed to engage participants in a comprehensive evaluation of their interactions with GitHub Copilot within their coding workflows. The process unfolds through a series of structured steps, each aimed at delving into different aspects of the user experience.

\paragraph{Step 1: Introduction to the Study}
The journey begins with a warm welcome to participants, setting the stage for a productive session. We provide them with an overview of the study's structure, which encompasses a warm-up session, contextual inquiry, and a concluding interview. Ensuring transparency and consent, we initiate the recording of the session via Zoom or Tencent Meeting to capture the nuances of each interaction.

\paragraph{Step 2: Warm-Up (5 Minutes)}
During the warm-up, participants are encouraged to open their Integrated Development Environment (IDE) and share a recent instance where they utilized Copilot for natural language-based code generation, rather than mere code completion. This segment is crucial for understanding their objectives, motivations for using Copilot, the approach adopted, and any challenges or friction points encountered during the process. Participants are asked to share their screens, and the session is recorded for in-depth analysis.

\paragraph{Step 3: Contextual Inquiry (30 Minutes)}
This phase invites participants to engage with one of their ongoing or chosen projects in real time. They are encouraged to experiment with Copilot features while articulating their thought process aloud. This 'think-aloud' method allows us to capture valuable insights into how participants interact with prompts, make modifications, and navigate through their coding tasks. Key observations and points of interest are noted for a more detailed discussion during the interview phase.

\paragraph{Step 4: Interview (20 Minutes)}
In the final segment, we revisit the points of interest identified during the contextual inquiry to delve deeper into the participant's experiences and perceptions. Time permitting, we expand the conversation to include broader questions about their overall experience with Copilot. This interview is also conducted through Zoom and is recorded to enrich our analysis.

This structured approach, conducted entirely via Zoom and meticulously recorded, ensures a comprehensive understanding of the participants' experiences with GitHub Copilot, from initial interactions to deeper, task-specific usage, culminating in reflective insights gathered during the interview stage. In cases where participants do not have an ongoing project, we may suggest revisiting a past commit on GitHub to simulate a continuation of their coding endeavors.

\subsubsection{Data Analysis}

In our study, the analysis of interview and session recording data was meticulously conducted by three co-authors through open coding, ensuring a thorough and unbiased interpretation of participant interactions with GitHub Copilot. We followed the thematic analysis~\cite{oktay2012grounded} method, specifically, we crafted a detailed codebook to categorize the prompt-result pairs demonstrated by participants, which allowed us to systematically identify patterns, challenges, and strategies within their usage of the AI assistant. Additionally, we tagged participants' statements to highlight specific themes and insights, further refining our analysis. This rigorous approach enabled us to distill complex data into meaningful findings, providing a deep understanding of how developers navigate and leverage the capabilities of AI-powered coding tools.

\subsection{Findings}

%% chatgpt


% F1 - observation: 
%     - abstraction level
%         - prompt scope
%     - prompt is a combination of text and code: 

%     F?
%     - contextual inquire -- using copilot in the wild: a large portion of code / entire project. Key takeaways?

%     - middle level - fuzzy + concrete, need an example to explain
%     - lack of code-prompt pairs
%     - lack of history
    
%  -- why / when to write prompt (fix errors, add input / output)
    
% F2 - pain points
%    - Lack of Instant Feedback (Slow feedback) / Controllability
%     - learning by error and trial - need iterations
    
%    - Huge code generated, regenerate from sketch, mess up
%    - Intensive Work of code + prompt combination
%     - scope control --> 
    
% F3 - Design Implication

\subsubsection{Coding with LLMs in The Wild: Scenarios \& Behaviors}

We observed distinct categorizations and behaviors among users engaging with coding assistant tools, specifically focusing on their tasks and coding expertise. Our contextual inquiry revealed a dichotomy in user needs based on their coding skills: experienced programmers (N = 5) often rely on automated code completion features to enhance productivity without overwhelming their codebase, valuing control and clarity in their coding process. Conversely, novices or those new to specific coding tasks (N = 6) showed a preference for using interactive chat features to navigate and understand coding practices more exploratively. When considering the nature of coding tasks, front-end developers emphasized code quality, prioritizing well-structured components, and refactoring, while algorithm developers concentrated on optimizing logic and efficiency, posing a challenge for the coding assistant's comprehension due to the abstract nature of these requirements. Feature usage patterns also emerged, with users employing strategies such as adding function inputs/outputs to prompts and enhancing function parameters for clearer guidance. Additionally, integrating web context into the coding assistant's workflow emerged as a valuable approach, where users first seek insights online before consulting the coding assistant, thereby enriching the context and improving the relevance of the assistant's suggestions.

\subsubsection{Prompts: Abstraction Levels}

Building on the insights from contextual inquiry, we further delved into the nuances of how users articulate their needs through prompts, a critical aspect of interacting with coding assistants. We categorized these prompts into three distinct abstraction levels: low, medium, and high, each reflecting a unique approach to communicating with the coding assistant. At the low abstraction level, users tend to provide the coding assistant with explicit commands or code snippets, leaving little to interpretation and ensuring a high degree of control over the output. Transitioning to the medium abstraction level, we observed a more intricate interplay between the user's intention and the inclusion of specific details. This is exemplified by prompts from participants like: ``Color scale based on ‘cluster’ column, 10 colors'' -- \textit{P10}, ``Plot the correlation between the top 10 features with highest correlation using a heat map, only showing top 10'' -- \textit{P1}. These prompts skillfully combine the what and the how, guiding the assistant while preserving the user's strategic goals. Conversely, some participants adopts an alternate medium-level strategy by outlining the technical specifics before revealing the broader objective, as seen in their prompt to ``Add parameters x / y to the function so that I can manage them'' -- \textit{P5}. At the high abstraction end, prompts are purely conceptual, focusing solely on the desired outcome without delving into the mechanics of implementation, challenging the assistant to interpret and execute the user's vision. The delineation of the medium abstraction level, however, posed a challenge, as the blending of intentions with varying degrees of detail resulted in a broad and sometimes ambiguous spectrum of user prompts, underscoring the diverse strategies employed by users to leverage coding assistants effectively within their unique coding contexts and tasks.


\subsubsection{Iterations: Learning by Trial and Error}

Building on our examination of how users navigate the abstraction levels in their prompts, our investigation extends into the iteration phase, which unveils the intricate dynamics of user engagement with coding assistants. We observed a significant investment of time and effort by participants, particularly when engaging in the iterative process of refining both prompts and the generated code. This process was notably pronounced at the middle and low levels of abstraction, where the balance between controlling the output and efficiently achieving desired results becomes a delicate dance. 

The quest for control over the coding assistant's output through prompt adjustments emerged as a formidable challenge, more so when users are faced with lengthy and complex code segments. This aspect of interaction becomes exceedingly strenuous at lower abstraction levels, where the precision in prompt crafting demands a substantial investment of time and cognitive effort. When the generated code deviates from the expected outcome, users find themselves ensnared in a time-consuming cycle of trial and error, attempting to refine prompts with the hope of steering the code generation closer to their desired intent. However, our observations indicate a pragmatic threshold among many participants (N=7), who exhibited a reluctance to exceed an average of 2 to 3 iterations of prompt modification. Beyond this point, the inclination shifts towards engaging directly with the code itself, opting for manual modifications over further prompt refinements. This transition from relying on the coding assistant's capabilities to applying personal coding acumen highlights a critical juncture in the iterative development process, illuminating the balance users strike between the convenience of automated assistance and the autonomy of hands-on code manipulation.

\subsubsection{Controllability: from Creative to Tedious}

We also delve into the dichotomy users face when interacting with large language models (LLMs) in coding tasks: the creative empowerment afforded by these models versus the potential tedium in achieving precise controllability. A significant hurdle in mastering controllability lies in the inherent difficulty of specifying the scope and extent of desired changes. The current mechanisms of auto-completion and inline chat offer limited avenues for users to convey comprehensive information and context to the model, thereby constraining their ability to direct its output accurately. Specifically, LLMs cannot provide instant feedback, like \textit{P10} said: ``If I could know what to change in the specific corresponding code while writing the prompt (in real-time), it would be useful in debug or learning code scenarios.''. This challenge is further exacerbated for users who may not possess the eloquence or experience to articulate their requirements effectively. Moreover, the pursuit of controllability transcends simple prompt adjustments, highlighting a complex interaction between the prompt's content and the broader context that is situated. Ideally, controllability should emerge from a harmonious blend of both of these elements. However, the absence of instant feedback mechanisms introduces a layer of opacity to the model's operational logic, leaving users to navigate a series of "black box" processes. This lack of transparency significantly impedes the user's capacity to influence the model's behavior in a predictable and desired manner.

As we culminate our findings, it's crucial to acknowledge that the challenges in achieving controllability may stem, in part, from the stochastic nature of LLMs themselves. The probabilistic and often unpredictable outputs generated by these models necessitate a more structured approach to prompting. To mitigate the inherent unpredictability and enhance user control, there's a pressing need for the development of structured rules and frameworks that can guide users in crafting their prompts. Such guidelines would not only facilitate more precise interactions with LLMs but also potentially alleviate the cognitive load on users, allowing them to delegate some of the model's tasks more effectively and efficiently. This shift towards a more rule-based prompting strategy underscores the ongoing evolution in our understanding and utilization of LLMs, particularly in the realm of coding and software development.



\subsection{Conclusion}

Our exploration into the interaction between users and large language models (LLMs) in coding contexts reveals a complex landscape marked by diverse user needs, the nuanced use of prompts, iterative refinement processes, and significant challenges in controllability. We observed a broad spectrum of user behaviors, from experienced programmers prioritizing control over their code to novices exploring coding concepts through interactive chats. The categorization of prompts into varying levels of abstraction highlighted the delicate balance users strive to achieve between specificity and generality, often leading to a labor-intensive cycle of trial and error as they seek to refine both prompts and the resulting code. This iterative process, while fostering a deeper understanding of the code, often culminates in a feeling of tedium and a lack of control, exacerbated by the stochastic nature of LLM outputs and the absence of instant feedback mechanisms. \textbf{These insights underscore the need for a transformative approach to LLM-assisted coding, one that integrates instant feedback and incremental prompt and code updates within a structured, interactive system.} By addressing these core issues, we can enhance the efficiency, controllability, and overall user experience of coding with LLMs, paving the way for more intuitive and empowering developer tools.

==> doc/_deprecated/3-formative_v1.tex <==

\section{Live Prompting for NL2Code}

Live Prompting supports
a short time span between a change to prompt 
and an observable change in the generated code

\subsection{Requirements of Live Prompting for NL2Code}

the deterministic 

immediate feedback

\begin{itemize}
    \item C1. The same prompt often leads to different outputs.
    This is two fold: 1) the ambiguity of prompt, and the LLMs non-deterministic natural.
    
    \item C2. The slow evaluation process of LLMs.
\end{itemize}

there is no a clear mapping between the user's prompt and the desired code,

the ambiguous process of transforming a programmer’s goal into generated code

ambiguity in user's prompt:
1) due to the ambiguity, there can be many outputs for the same input
2) due to the ambiguity, we need LLM to understand it.

In what cases the user's prompt would be determinist?

% Live programming is a paradigm in which, given a context, immediate feedback on program
% execution is always provided to the programmer
% support live programming through

When every evaluating a state
- the same state should lead to the same output
- it should be fast
- output?


\subsection{Formative Study}
We need a study to understand if, and when there is a clear mapping between the user's prompt and desired code.

% To better understand the real difficulties encountered by users when coding with LLM, 
% we conducted a contextual inquiry (specifically focusing on GitHub Copilot) as a formative study, 
% in which we observed in detail how users interact with LLM when they are not involved in an in-lab controlled coding task.

\subsection{Study Setup}
% - participants
% - procedure
% - analysis

\paragraph{Participants.}
We recruited 11 participants through university mailing lists and forums, selecting them based on a screening questionnaire that assessed programming proficiency and experience with AI Coding Assistants (e.g., GitHub Copilot or ChatGPT). 
Our focus was on individuals who utilized textual prompts to guide AI models in coding tasks, 
excluding those who solely relied on the auto-complete feature of these models. 
Participants were required to present a recent project where they employed LLMs for coding. 
Participant backgrounds are detailed in Table~\ref{table: formative participants}.

\begin{table}[!tbh]
\resizebox{\linewidth}{!}{
\begin{tabular}{cccl}
\toprule
    & \textbf{Years on Coding} & \textbf{Frequency of using LLMs} & \textbf{Project Type}                    \\ \midrule
P1  & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P2  & 5+                            & Daily                        & Front-end Development          \\ \hline
P3  & 5+                            & Always                       & Front-end Development          \\ \hline
P4  & 5+                            & Always                       & Machine Learning                    \\ \hline
P5  & 5+                            & Monthly                      & Back-end Development           \\ \hline
P6  & 3-5                           & Daily                           & Back-end Development            \\ \hline
P7  & 3-5                           &  Always                       & Machine Learning                    \\ \hline
P8  & 5+                            &  Always                        &  Front-end Development        \\ \hline
P9  & 5+                              &  Daily                            &  Front-end Development      \\ \hline
P10 & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P11 & 1-2                           &  Weekly                            & Embedded Systems Development    \\ \hline
\end{tabular}
}

\caption{Participants in Formative Study}
\label{table: formative participants}
\end{table}

\paragraph{Procedure.}
Our study is designed to understand how participants interact with LLMs within their coding workflows. 
The study is structured into a warm-up session (5mins), a contextual inquiry(30mins), and a final interview (20mins).
In the warm-up phase, participants open their IDE and share a recent experience using LLMs for code generation beyond simple code completion. 
Following the warm-up is a contextual inquiry.
Participants work on an ongoing project, using LLMs while verbalizing their thought process. 
% This `think-aloud' technique gives us direct insight into their interactions, adjustments, and decision-making as they code. 
We note observations for further exploration in the interview phase.
The study concludes with an interview, 
diving into the experiences and perceptions highlighted during the inquiry. 
We also discuss their overall experience with LLMs to gather comprehensive feedback. 
This interview is conducted via Zoom and recorded (both video and audio) for analysis.
Participants provided consent and were compensated with \$20 for the 60-minute session.

\paragraph{Data Analysis.}
The interviews were audio-recorded, transcribed, and independently coded by three co-authors. Discrepancies in coding were resolved through discussion. 
Additionally, we collected and examined the prompts used by participants, as well as the corresponding code generated during the contextual inquiry, using the video recordings to deepen our understanding of the exact text used by the participants and its context.
Our analysis employed the thematic analysis method, generating the codes and themes both 
 both inductively (i.e., bottom-up) and deductively (i.e., topdown),
The final themes were established after three rounds of iterative refinement.

\subsection{Findings \zt{WIP}}

\textbf{explicitly refer to existing codes.}
\textbf{explicitly refer to external codes.}
\textbf{implicitly refer to codes.}

%% chatgpt


% F1 - observation: 
%     - abstraction level
%         - prompt scope
%     - prompt is a combination of text and code: 

%     F?
%     - contextual inquire -- using copilot in the wild: a large portion of code / entire project. Key takeaways?

%     - middle level - fuzzy + concrete, need an example to explain
%     - lack of code-prompt pairs
%     - lack of history
    
%  -- why / when to write prompt (fix errors, add input / output)
    
% F2 - pain points
%    - Lack of Instant Feedback (Slow feedback) / Controllability
%     - learning by error and trial - need iterations
    
%    - Huge code generated, regenerate from sketch, mess up
%    - Intensive Work of code + prompt combination
%     - scope control --> 
    
% F3 - Design Implication

\subsubsection{Coding with LLMs in The Wild: Scenarios \& Behaviors}

We observed distinct categorizations and behaviors among users engaging with coding assistant tools, specifically focusing on their tasks and coding expertise. 
Our contextual inquiry revealed a dichotomy in user needs based on their coding skills: experienced programmers (N = 5) often rely on automated code completion features to enhance productivity without overwhelming their codebase, valuing control and clarity in their coding process. 
Conversely, novices or those new to specific coding tasks (N = 6) showed a preference for using interactive chat features to navigate and understand coding practices more exploratively. 
When considering the nature of coding tasks, front-end developers emphasized code quality, prioritizing well-structured components, and refactoring, while algorithm developers concentrated on optimizing logic and efficiency, posing a challenge for the coding assistant's comprehension due to the abstract nature of these requirements. 
Feature usage patterns also emerged, with users employing strategies such as adding function inputs/outputs to prompts and enhancing function parameters for clearer guidance. 
Additionally, integrating web context into the coding assistant's workflow emerged as a valuable approach, where users first seek insights online before consulting the coding assistant, thereby enriching the context and improving the relevance of the assistant's suggestions.

\subsubsection{Prompts: Abstraction Levels}

Building on the insights from contextual inquiry, we further delved into the nuances of how users articulate their needs through prompts, a critical aspect of interacting with coding assistants. We categorized these prompts into three distinct abstraction levels: low, medium, and high, each reflecting a unique approach to communicating with the coding assistant. At the low abstraction level, users tend to provide the coding assistant with explicit commands or code snippets, leaving little to interpretation and ensuring a high degree of control over the output. Transitioning to the medium abstraction level, we observed a more intricate interplay between the user's intention and the inclusion of specific details. This is exemplified by prompts from participants like: ``Color scale based on ‘cluster’ column, 10 colors'' -- \textit{P10}, ``Plot the correlation between the top 10 features with highest correlation using a heat map, only showing top 10'' -- \textit{P1}. These prompts skillfully combine the what and the how, guiding the assistant while preserving the user's strategic goals. Conversely, some participants adopts an alternate medium-level strategy by outlining the technical specifics before revealing the broader objective, as seen in their prompt to ``Add parameters x / y to the function so that I can manage them'' -- \textit{P5}. At the high abstraction end, prompts are purely conceptual, focusing solely on the desired outcome without delving into the mechanics of implementation, challenging the assistant to interpret and execute the user's vision. The delineation of the medium abstraction level, however, posed a challenge, as the blending of intentions with varying degrees of detail resulted in a broad and sometimes ambiguous spectrum of user prompts, underscoring the diverse strategies employed by users to leverage coding assistants effectively within their unique coding contexts and tasks.


\subsubsection{Iterations: Learning by Trial and Error}

Building on our examination of how users navigate the abstraction levels in their prompts, our investigation extends into the iteration phase, which unveils the intricate dynamics of user engagement with coding assistants. We observed a significant investment of time and effort by participants, particularly when engaging in the iterative process of refining both prompts and the generated code. This process was notably pronounced at the middle and low levels of abstraction, where the balance between controlling the output and efficiently achieving desired results becomes a delicate dance. 

The quest for control over the coding assistant's output through prompt adjustments emerged as a formidable challenge, more so when users are faced with lengthy and complex code segments. This aspect of interaction becomes exceedingly strenuous at lower abstraction levels, where the precision in prompt crafting demands a substantial investment of time and cognitive effort. When the generated code deviates from the expected outcome, users find themselves ensnared in a time-consuming cycle of trial and error, attempting to refine prompts with the hope of steering the code generation closer to their desired intent. However, our observations indicate a pragmatic threshold among many participants (N=7), who exhibited a reluctance to exceed an average of 2 to 3 iterations of prompt modification. Beyond this point, the inclination shifts towards engaging directly with the code itself, opting for manual modifications over further prompt refinements. This transition from relying on the coding assistant's capabilities to applying personal coding acumen highlights a critical juncture in the iterative development process, illuminating the balance users strike between the convenience of automated assistance and the autonomy of hands-on code manipulation.



\subsubsection{Controllability: from Creative to Tedious}


We also delve into the dichotomy users face when interacting with large language models (LLMs) in coding tasks: the creative empowerment afforded by these models versus the potential tedium in achieving precise controllability. A significant hurdle in mastering controllability lies in the inherent difficulty of specifying the scope and extent of desired changes. The current mechanisms of auto-completion and inline chat offer limited avenues for users to convey comprehensive information and context to the model, thereby constraining their ability to direct its output accurately. Specifically, LLMs cannot provide instant feedback, like \textit{P10} said: ``If I could know what to change in the specific corresponding code while writing the prompt (in real-time), it would be useful in debug or learning code scenarios.''. This challenge is further exacerbated for users who may not possess the eloquence or experience to articulate their requirements effectively. Moreover, the pursuit of controllability transcends simple prompt adjustments, highlighting a complex interaction between the prompt's content and the broader context that is situated. Ideally, controllability should emerge from a harmonious blend of both of these elements. However, the absence of instant feedback mechanisms introduces a layer of opacity to the model's operational logic, leaving users to navigate a series of "black box" processes. This lack of transparency significantly impedes the user's capacity to influence the model's behavior in a predictable and desired manner.

As we culminate our findings, it's crucial to acknowledge that the challenges in achieving controllability may stem, in part, from the stochastic nature of LLMs themselves. The probabilistic and often unpredictable outputs generated by these models necessitate a more structured approach to prompting. To mitigate the inherent unpredictability and enhance user control, there's a pressing need for the development of structured rules and frameworks that can guide users in crafting their prompts. Such guidelines would not only facilitate more precise interactions with LLMs but also potentially alleviate the cognitive load on users, allowing them to delegate some of the model's tasks more effectively and efficiently. This shift towards a more rule-based prompting strategy underscores the ongoing evolution in our understanding and utilization of LLMs, particularly in the realm of coding and software development.



\subsection{Conclusion}

\newpage
% Our exploration into the interaction between users and large language models (LLMs) in coding contexts reveals a complex landscape marked by diverse user needs, the nuanced use of prompts, iterative refinement processes, and significant challenges in controllability. We observed a broad spectrum of user behaviors, from experienced programmers prioritizing control over their code to novices exploring coding concepts through interactive chats. The categorization of prompts into varying levels of abstraction highlighted the delicate balance users strive to achieve between specificity and generality, often leading to a labor-intensive cycle of trial and error as they seek to refine both prompts and the resulting code. This iterative process, while fostering a deeper understanding of the code, often culminates in a feeling of tedium and a lack of control, exacerbated by the stochastic nature of LLM outputs and the absence of instant feedback mechanisms. \textbf{These insights underscore the need for a transformative approach to LLM-assisted coding, one that integrates instant feedback and incremental prompt and code updates within a structured, interactive system.} By addressing these core issues, we can enhance the efficiency, controllability, and overall user experience of coding with LLMs, paving the way for more intuitive and empowering developer tools.

==> doc/_deprecated/3-formative_v2.tex <==

\section{Understanding Direct Code References in Prompts}

The goal of this work is to investigate the utilization of linguistic structures inherent in prompts for transforming them into code sketches. 
Central to this language-oriented approach is identifying the correspondences between phrases within the prompt and elements of the code. 
We refer a word or phrase within a prompt as a \emph{Code Reference}
if it specifically points to a piece of code (formally a node on the Abstract Syntax Tree~\cite{}).
These phrase-level references serve as anchor points, linking the prompt's linguistic structure to specific code elements, and play a crucial role to achieve our goal since we aim to update the code sketch incrementally as the user types.
\zt{why? should justify more}

To inform our approach, we conducted a contextual inquire aimed at understanding the reasons, 
methods, 
and contexts in which users employ code references in their prompts. 

% Examples of DCR:
% "Initialize an integer variable named counter."

% DCR: "integer variable" and "counter." The phrase "integer variable" directly refers to the type of variable to be declared in the code, and "counter" specifies its name, directly mapping to a variable declaration in the code, such as int counter; in C++ or Java.
% "Call the sortByDate function with the events array as an argument."

% DCR: "sortByDate function" and "events array." "sortByDate function" directly points to a specific function in the code, and "events array" refers to a particular array, indicating an actual function call, e.g., sortByDate(events);.
% "Implement a for loop to iterate over items."

% DCR: "for loop" and "items." The term "for loop" indicates a specific control flow structure, and "items" suggests an iterable variable in the code, corresponding to a construct like for(item in items){...}.
% Examples of Non-DCR:
% "Ensure the application scales efficiently."

% This sentence does not directly reference a specific piece of code or an AST node. Instead, it describes a high-level requirement or goal, focusing on the application's behavior rather than its implementation.
% "Optimize the algorithm for faster computation."

% Similar to the previous example, this directive is about enhancing performance but does not specify any direct code construct, function, or variable to modify. It’s more about the approach or methodology rather than a direct code element.
% "Use a secure method for data encryption."

% While "data encryption" hints at a general task or functionality, it does not specify a direct code referent such as a specific encryption function or library to be used in the code. It's a broader directive that can be implemented through various code solutions.
% In summary, a Direct Code Referent (DCR) is explicitly tied to identifiable code elements or constructs, such as variables, functions, loops, or data structures, as mentioned in a natural language description. Conversely, statements that outline general goals, non-specific methodologies, or conceptual strategies without directly pointing to specific code elements do not contain DCRs.


% To better understand the real difficulties encountered by users when coding with LLM, 
% we conducted a contextual inquiry (specifically focusing on GitHub Copilot) as a formative study, 
% in which we observed in detail how users interact with LLM when they are not involved in an in-lab controlled coding task.

\subsection{Study Setup}
% - participants
% - procedure
% - analysis

\paragraph{Participants.}
We recruited 11 participants through university mailing lists and forums, selecting them based on a screening questionnaire that assessed programming proficiency and experience with AI Coding Assistants (e.g., GitHub Copilot or ChatGPT). 
Our focus was on individuals who utilized textual prompts to guide AI models in coding tasks, 
excluding those who solely relied on the auto-complete feature of these models. 
Participants were required to present a recent project where they employed LLMs for coding. 
Participant backgrounds are detailed in Table~\ref{table: formative participants}.

\begin{table}[!tbh]
\resizebox{\linewidth}{!}{
\begin{tabular}{cccl}
\toprule
    & \textbf{Years on Coding} & \textbf{Frequency of using LLMs} & \textbf{Project Type}                    \\ \midrule
P1  & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P2  & 5+                            & Daily                        & Front-end Development          \\ \hline
P3  & 5+                            & Always                       & Front-end Development          \\ \hline
P4  & 5+                            & Always                       & Machine Learning                    \\ \hline
P5  & 5+                            & Monthly                      & Back-end Development           \\ \hline
P6  & 3-5                           & Daily                           & Back-end Development            \\ \hline
P7  & 3-5                           &  Always                       & Machine Learning                    \\ \hline
P8  & 5+                            &  Always                        &  Front-end Development        \\ \hline
P9  & 5+                              &  Daily                            &  Front-end Development      \\ \hline
P10 & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P11 & 1-2                           &  Weekly                            & Embedded Systems Development    \\ \hline
\end{tabular}
}

\caption{Participants in Formative Study}
\label{table: formative participants}
\end{table}

\paragraph{Procedure.}
Our study is designed to understand how participants interact with LLMs within their coding workflows. 
The study is structured into a warm-up session (5mins), a contextual inquiry(30mins), and a final interview (20mins).
In the warm-up phase, participants open their IDE and share a recent experience using LLMs for code generation beyond simple code completion. 
Following the warm-up is a contextual inquiry.
Participants work on an ongoing project, using LLMs while verbalizing their thought process. 
% This `think-aloud' technique gives us direct insight into their interactions, adjustments, and decision-making as they code. 
We note observations for further exploration in the interview phase.
The study concludes with an interview, 
diving into the experiences and perceptions highlighted during the inquiry. 
We also discuss their overall experience with LLMs to gather comprehensive feedback. 
This interview is conducted via Zoom and recorded (both video and audio) for analysis.
Participants provided consent and were compensated with \$20 for the 60-minute session.

\paragraph{Data Analysis.}
The interviews were audio-recorded, transcribed, and independently coded by three co-authors. Discrepancies in coding were resolved through discussion. 
Additionally, we collected and examined the prompts used by participants, as well as the corresponding code generated during the contextual inquiry, using the video recordings to deepen our understanding of the exact text used by the participants and its context.
Our analysis employed the thematic analysis method, generating the codes and themes both 
 both inductively (i.e., bottom-up) and deductively (i.e., topdown),
The final themes were established after three rounds of iterative refinement.

\subsection{Findings \zt{WIP}}

% \subsubsection{Coding with LLMs in The Wild: Scenarios \& Behaviors}

% We observed distinct categorizations and behaviors among users engaging with coding assistant tools, specifically focusing on their tasks and coding expertise. 
% Our contextual inquiry revealed a dichotomy in user needs based on their coding skills: experienced programmers (N = 5) often rely on automated code completion features to enhance productivity without overwhelming their codebase, valuing control and clarity in their coding process. 
% Conversely, novices or those new to specific coding tasks (N = 6) showed a preference for using interactive chat features to navigate and understand coding practices more exploratively. 
% When considering the nature of coding tasks, front-end developers emphasized code quality, prioritizing well-structured components, and refactoring, while algorithm developers concentrated on optimizing logic and efficiency, posing a challenge for the coding assistant's comprehension due to the abstract nature of these requirements. 
% Feature usage patterns also emerged, with users employing strategies such as adding function inputs/outputs to prompts and enhancing function parameters for clearer guidance. 
% Additionally, integrating web context into the coding assistant's workflow emerged as a valuable approach, where users first seek insights online before consulting the coding assistant, thereby enriching the context and improving the relevance of the assistant's suggestions.

\subsubsection{Users refer to code because xxx}

% Users refer to code elements in their prompts primarily to bridge the gap between natural language instructions and the precise, structured requirements of programming languages. This practice stems from the need to communicate complex programming concepts and intentions succinctly and accurately to LLMs. By embedding specific code elements within their prompts, users aim to:

% - Increase Precision: Direct references to code elements help ensure that the generated code aligns closely with the user's specific requirements, minimizing ambiguity.
% - Guide Code Generation (Controllability): These references act as anchors or waypoints for the LLM, guiding the code generation process towards the desired structure and functionality.
% - Facilitate Understanding: For users themselves, incorporating code elements in prompts helps clarify their own thinking, making the abstraction more tangible.
% - Lack of other methods (no other UI methods to refer code)


% A significant hurdle in mastering controllability lies in the inherent difficulty of specifying the scope and extent of desired changes. The current mechanisms of auto-completion and inline chat offer limited avenues for users to convey comprehensive information and context to the model, thereby constraining their ability to direct its output accurately. Specifically, LLMs cannot provide instant feedback, like \textit{P10} said: ``If I could know what to change in the specific corresponding code while writing the prompt (in real-time), it would be useful in debug or learning code scenarios.''. This challenge is further exacerbated for users who may not possess the eloquence or experience to articulate their requirements effectively. Moreover, the pursuit of controllability transcends simple prompt adjustments, highlighting a complex interaction between the prompt's content and the broader context that is situated. Ideally, controllability should emerge from a harmonious blend of both of these elements. However, the absence of instant feedback mechanisms introduces a layer of opacity to the model's operational logic, leaving users to navigate a series of "black box" processes. This lack of transparency significantly impedes the user's capacity to influence the model's behavior in a predictable and desired manner.

% As we culminate our findings, it's crucial to acknowledge that the challenges in achieving controllability may stem, in part, from the stochastic nature of LLMs themselves. The probabilistic and often unpredictable outputs generated by these models necessitate a more structured approach to prompting. To mitigate the inherent unpredictability and enhance user control, there's a pressing need for the development of structured rules and frameworks that can guide users in crafting their prompts. Such guidelines would not only facilitate more precise interactions with LLMs but also potentially alleviate the cognitive load on users, allowing them to delegate some of the model's tasks more effectively and efficiently. This shift towards a more rule-based prompting strategy underscores the ongoing evolution in our understanding and utilization of LLMs, particularly in the realm of coding and software development.


\subsubsection{Mechanisms of Direct Code References in Prompts}

In analyzing how participants refer to code in their prompts, 
we identify two types of references: \emph{independent} and \emph{dependent}.

\begin{itemize}[leftmargin=*]
    \item \emph{Independent Reference} standalone points to code elements, typically employing the exact identifier of these elements (e.g., variable or function names) or reserved keywords. 
    The code referent of an independent reference can be precisely located without extra contextual information in the prompt. 
    For example, \zt{example} \textcolor{red}{(1) Converts $t_x$ and $t_y$ to pixel-based coordinates, (2) print the shape of $SalePrice$ in train.csv, (3) start reading data when you see \$ sign, stop reading data when you see \# sign, etc.}
    % when a participant uses "Initialize array dataStorage", "array" acts as an independent reference. The term directly points to a specific code construct, and dataStorage identifies the exact variable involved, allowing for clear and immediate identification within the codebase.
     \textcolor{red}{Edit code \textbf{above}; Add \textbf{this}, with model save name automated; the return type of \textbf{this} function is a node list }
     \textcolor{red}{\textbf{write} data to the serial port; \textbf{Convert} the string data to floating-point numbers}

    \item \emph{Dependent Reference}, on the other hand, refers to code elements through their relationship with other references within the prompt.
    The code referent of a dependent reference cannot be accurately located without additional information provided by the surrounding text.
    For example, \zt{example}
    % The referent of "it" (i.e., the array dataStorage) is understood only by considering its relationship with the independent reference that precedes it.
\end{itemize}

Identifying how a reference refer to code helps in developing strategies for parsing prompts as the user types and mapping them to code elements.

% if a participant mentions "Call the fetchUserData function with a timeout of 5000 milliseconds," the phrase explicitly refers to a function named fetchUserData. 
% These references are usually nouns as symbols.
% direct mention similar to the mathmatical symbols in text.

% Implicit DCRs, in contrast, depend on their linguistic relationship with other DCRs in the prompt to point toward code elements.
% Typical examples include:
% 1) pronoun (e.g., \zt{example}), 
% 2) verb (\emph{example} ),
% 3) dobj
% In summary, an implicit DCR itself cannot refer to a code element.
% However, we can resolve its code referent based on its relationsihp with other DCR.
% For instance, a statement like "Ensure the data fetching process is asynchronous" employs an implicit DCR for describing a feature of the code (asynchronous data fetching). Here, "data fetching process" implies a function or method responsible for retrieving data, and "asynchronous" suggests how this process should be executed, even though no specific function name or variable is mentioned.

% This distinction between explicit and implicit DCRs aids in identifying whether a phrase typed by a user is directly referring to a piece of code or if it indicates code through linguistic associations. 
% Recognizing this difference is crucial for developing our approach.

% In their prompts, participants refereed to code either \emph{explicitly} or \emph{implicitly}.
% In our study, we found that \zt{some data}.

% Explicit DCRs refer to code directly using the identical identifier of the code elements, such as 
% variable names, function names, or even inline codes,
% and can be directly mapped to code constructs without additional contextual information. 
% For example, \zt{xxxx need an example.}

% On the other hand, implicit DCRs, refer to code rely on their linguistic relationship with other explict DCRs in the prompt.
% For example, \zt{xxx an example.}

% This distinction helps us understand how to detect if a typing phrase is a DCR or not.

\subsubsection{Context of Code References: An Intermediate Level of Clarity}
In our study, we found that users often refer to code elements when they possess an intermediate level of clarity about the desired code.
Previous research~\cite{} has categorized user interactions with LLM-based programming assistants into two modes: acceleration, characterized by a clear vision of the intended code, and exploration, marked by uncertainty about the solution. 
Our observations echo these distinctions, 
revealing that users in exploration mode often 
describe their problems rather than specify code elements, 
utilizing tools like ChatGPT or Copilot Chat for guidance. 
Conversely, those in acceleration mode lean towards direct code manipulation, 
favoring features like Copilot's auto-completion instead of NL prompts.

In addition to exploration and acceleration mode,
we also noticed that participants often have an intermediate clarity of the intended code -- a state where the user possesses an overall conceptions of the necessary functions, variables, or code structures but lacks confidence in the finer details.  
For instance, a user might request the creation of a \emph{``REST API with a GET handler to read from a database''}, 
implying a clear idea of the desired code element (i.e., \emph{a GET handler}) 
reveals ambiguity about how to achieve this functionality (i.e., how to \emph{read from a database}).
This intermediary position encourages more frequent referencing of code elements as users seek to align the generated code with their project's architectural goals and details.
In this intermediate clarity zone, 
participants find Copilot Inline Chat or inline comments to be more suitable.

It's crucial to acknowledge that our classification of user behavior represents a spectrum rather than discrete categories. Users dynamically transition among these states throughout the coding process, reflecting the fluid and dynamic nature of software development.
These observations not only highlight the versatility required of LLM-based programming assistants 
but also pinpoint the specific scenario where our Language-Oriented Code Sketching approach can offer the most value.



% \subsubsection{Prompts: Abstraction Levels}
%Transitioning to the medium abstraction level, we observed a more intricate interplay between the user's intention and the inclusion of specific details. This is exemplified by prompts from participants like: ``Color scale based on ‘cluster’ column, 10 colors'' -- \textit{P10}, ``Plot the correlation between the top 10 features with highest correlation using a heat map, only showing top 10'' -- \textit{P1}. These prompts skillfully combine the what and the how, guiding the assistant while preserving the user's strategic goals. Conversely, some participants adopts an alternate medium-level strategy by outlining the technical specifics before revealing the broader objective, as seen in their prompt to ``Add parameters x / y to the function so that I can manage them'' -- \textit{P5}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% F1 - observation: 
%     - abstraction level
%         - prompt scope
%     - prompt is a combination of text and code: 

%     F?
%     - contextual inquire -- using copilot in the wild: a large portion of code / entire project. Key takeaways?

%     - middle level - fuzzy + concrete, need an example to explain
%     - lack of code-prompt pairs
%     - lack of history
    
%  -- why / when to write prompt (fix errors, add input / output)
    
% F2 - pain points
%    - Lack of Instant Feedback (Slow feedback) / Controllability
%     - learning by error and trial - need iterations
    
%    - Huge code generated, regenerate from sketch, mess up
%    - Intensive Work of code + prompt combination
%     - scope control --> 
    
% F3 - Design Implication


% \subsubsection{Iterations: Learning by Trial and Error}

% Building on our examination of how users navigate the abstraction levels in their prompts, our investigation extends into the iteration phase, which unveils the intricate dynamics of user engagement with coding assistants. We observed a significant investment of time and effort by participants, particularly when engaging in the iterative process of refining both prompts and the generated code. This process was notably pronounced at the middle and low levels of abstraction, where the balance between controlling the output and efficiently achieving desired results becomes a delicate dance. 

% The quest for control over the coding assistant's output through prompt adjustments emerged as a formidable challenge, more so when users are faced with lengthy and complex code segments. This aspect of interaction becomes exceedingly strenuous at lower abstraction levels, where the precision in prompt crafting demands a substantial investment of time and cognitive effort. When the generated code deviates from the expected outcome, users find themselves ensnared in a time-consuming cycle of trial and error, attempting to refine prompts with the hope of steering the code generation closer to their desired intent. However, our observations indicate a pragmatic threshold among many participants (N=7), who exhibited a reluctance to exceed an average of 2 to 3 iterations of prompt modification. Beyond this point, the inclination shifts towards engaging directly with the code itself, opting for manual modifications over further prompt refinements. This transition from relying on the coding assistant's capabilities to applying personal coding acumen highlights a critical juncture in the iterative development process, illuminating the balance users strike between the convenience of automated assistance and the autonomy of hands-on code manipulation.







\subsection{Conclusion}

\newpage
% Our exploration into the interaction between users and large language models (LLMs) in coding contexts reveals a complex landscape marked by diverse user needs, the nuanced use of prompts, iterative refinement processes, and significant challenges in controllability. We observed a broad spectrum of user behaviors, from experienced programmers prioritizing control over their code to novices exploring coding concepts through interactive chats. The categorization of prompts into varying levels of abstraction highlighted the delicate balance users strive to achieve between specificity and generality, often leading to a labor-intensive cycle of trial and error as they seek to refine both prompts and the resulting code. This iterative process, while fostering a deeper understanding of the code, often culminates in a feeling of tedium and a lack of control, exacerbated by the stochastic nature of LLM outputs and the absence of instant feedback mechanisms. \textbf{These insights underscore the need for a transformative approach to LLM-assisted coding, one that integrates instant feedback and incremental prompt and code updates within a structured, interactive system.} By addressing these core issues, we can enhance the efficiency, controllability, and overall user experience of coding with LLMs, paving the way for more intuitive and empowering developer tools.

==> doc/draft/1-intro_v1.tex <==
\section{Introduction}

The advent of Large Language Models (LLMs) represents a paradigm shift in programming, 
enabling an era where natural language (NL) prompts can directly inform code generation and editing~\cite{}. 
Despite this advancement, % is groundbreaking, 
programmers frequently encounter a tedious loop of trial and error, continuously refining their prompts to guide LLMs to the desired code, e.g., as shown in user testing of SYSTEM NAME~\cite{}.
Existing solutions, 
such as Grounded Abstraction Matching~\cite{} 
and interactive systems that guide the decomposition of complex prompts into detailed sub-prompts~\cite{}, 
while useful, 
fall short in providing immediate feedback during the prompt crafting process. 
The lack of such feedback can lead to uncertainty about the expected output, 
decreased user engagement, 
and potential inefficiencies in the development process, 
as users are left to mentally imagine possible outcomes until the code is generated~\cite{}.

However, providing immediate feedback during prompt crafting presents significant challenges.
Ideally, feedback should not only be \emph{instant} but also evolve \emph{incrementally} as the user types their prompt, 
offering clear and understandable intermediate results that progressively guide \zt{whom?} toward the final desired code.
The most straightforward approach—continuously sending the user's prompt to LLMs for feedback—is currently impractical, due to the computational demands and the unpredictable nature of LLM outputs, 
which can vary greatly as the prompt evolves~\cite{}.
These limitations highlight the need for innovative approaches that extend beyond mere reliance on LLMs.
%, potentially leveraging hybrid models or heuristic-based mechanisms to bridge this gap.

One observation, however, is that users' prompts frequently include phrases directly referencing code elements, embedded within narratives that reflect the relationships among these elements in the intended code structure.
For example, consider the prompt \emph{``Define a Pytorch dataset with a loadImg function''} (\autoref{fig:teaser}a).
Here, \colorbox{mypink}{\texttt{Pytorch dataset}} and \colorbox{mypink}{\texttt{loadImg function}} reference a class and a function, respectively.
Their linguistic relationship -- where \\ \colorbox{mypink}{\texttt{loadImg function}} is a child of \colorbox{mypink}{\texttt{Pytorch dataset}} associated through \emph{``with''} -- reveals that the function is meant to be a component of the class.
This linguistic structure of the prompt offers an interesting opportunity to create a \emph{code sketch} (i.e., an incomplete code outline~\cite{}) 
by mapping these phrases to predefined code snippets and then assembling them based on their linguistic relationship.
The resultant sketch (\autoref{fig:teaser}b) not only offer a preview of the intended code structure of the prompt,
but also serves as a foundational layer for LLMs to further refine and complete (\autoref{fig:teaser}c), 
thereby facilitating the interaction between programmers and LLMs. 
Moreover, such a process can be achieved by using classic natural language processing (NLP) techniques, 
bypassing the constraints inherent in solutions based solely on LLMs.


This work thus explores using the linguistic structure within prompts
% how the linguistic structure within prompts 
% can be used 
to instantly and incrementally create code sketches.
We focus on the scenarios where users use natural language prompts to generate or edit codes through LLMs.\zt{to be finished}
% We first conducted a formative study to understand why, how, and when users reference code in their prompts.
% The finding reveals that \zt{xxxx}.
% Informed by the study,
We design \emph{Language-Oriented Code Sketching}, 
an interactive approach that converts a prompt to a code sketch as the user is typing.
Through a user interface of auto-completion,
this method converts a prompt to a code sketch instantly and incrementally
without taxing users extra cognitive loads, also allowing users to interactively solving the ambiguities of the natural language.
We implement our approach in a proof-of-concept system, with a set of novel interactive features, and report a comparative study
on the use of the system as a technology probe~\cite{}
to understand how Language-Oriented Code Sketching
facilitate human-AI coding.
The result shows that \zt{xxxx}.

Contribution:
\begin{itemize}
    \item an approach, \method{}, that convert prompts to code sketch instantly and incrementally.
    \item a proof-of-concept system as a technology probe that implements the \method{}, as well as a set of novel interactive features to facilitate human-AI collaborations in programming.
    \item an evaluation xxx
\end{itemize}

% Such a sketch not only aids further refinement but also enhances the interaction between the programmer and LLM by 
% providing a tangible blueprint that evolves in real-time with the user's input.
% The key philosopy, is that before building the big thing, we incrementally move small steps, and intemediate results.
% \emph{immediate, incremental feedback} is given with each modification of the prompt, potentially including generated code or other valuable intermediate results.



% Many existing methods attempt to bridge the abstraction gap by 
% helping users write more effective prompts~\cite{}.
% For example, Liu et al. introduced the
% technique of grounded abstraction matching, 
% which involves translating the code back into a NL expression which can be edited and used for futher iterations.
% Another major approach is to decompose complex prompts into sub-prompts
% of a pre-defined abstraction level~\cite{}. Specifically,
% the programming task is divided into smaller, more manageable
% sub-tasks, each at a set level of complexity or detail.
% Despite the value of these methods, 
% these solutions still rely heavily on LLMs to provide feedback. 
% still, they all require users to directly interact with LLMs, and need to wait for a long time to see the generated code as feedback.

% While there have been efforts within the domain to mitigate these challenges—ranging from techniques aimed at refining user prompts to strategies for decomposing complex tasks into simpler sub-prompts—these solutions still rely heavily on LLMs to provide feedback. 
% Such reliance not only sustains the feedback delay but also underscores the limitations of existing methodologies in offering a swift, interactive coding experience. 
% Moreover, though incremental code generation using LLMs has been explored, 
% the fundamental bottleneck of slow feedback remains unaddressed, 
% given the computational intensity and unpredictability of LLM outputs.



% This methodology, which we term \emph{Incremental Code Sketching (ICS)}, serves as a bridge between the user's conceptual intent and the LLM's powerful code generation capabilities. 
% By providing users with an immediate sketch of their code, we facilitate a dynamic dialogue between the programmer and the LLM. 
% This not only streamlines the coding process but also mitigates the cognitive load on the user, making the interaction with LLMs more intuitive and productive. 
% Through ICS, we leverage the strengths of LLMs for detailed, sophisticated code generation while addressing their limitations in speed and interactivity, presenting a balanced approach to modern coding challenges.

% ICS acts as a conduit between the user's conceptual intent and the LLM's robust code generation capabilities, fostering a dynamic exchange that reduces cognitive load and enhances productivity. By offering an immediate representation of the user's idea, ICS leverages LLMs' strengths in generating detailed code while addressing their limitations in responsiveness and user interaction, thus offering a nuanced solution to contemporary programming challenges.

% Imagine a paradigm shift towards \emph{``Live Prompting''} — a notion inspired by ``Live Programming''~\cite{}.
% In this envisioned scenario, 
% \emph{immediate, incremental feedback} is given with each modification of the prompt, potentially including generated code or other valuable intermediate results.
% This feedback mechanism facilitate a smoother transition from prompt to  code, reducing the trial-and-error cycle. 
% However, achieving Live Prompting presents significant challenges.
% Continuously evaluating the user's prompt using LLMs as they type may not be a feasible solution, at least currently, due to the computational intensity and inherent unpredictability of LLM outputs. 
% These constraints necessitate innovative approaches to realize the notion of Live Prompting beyond solely LLM reliance.

% they confront a fundamental problem: 
% the slow feedback loop.
% The delay between writing a prompt, submitting it, awaiting the generated code, and then evaluating the code undermines productivity and escalates frustration. 
% This latency is a direct consequence of the computational demands of LLMs coupled with the iterative refinement process.


%% LLM for coding is good, what it is? NLP --> Code

%% despite the good, it sucks. it sucks in multiple way, feedback is slow and huge, lacking of controllability.

%% Option2: To tackle these issues, we aim to provide instant, incremental feedback when the user is typing prompt.
%% we achieve this by leveraging the embedded structure in the prompt.

%% we propose a xx method. how applicable of our method.

%% our method is awesome.
%% Additionally, enable a set of new interactions and UX.

%% through a user study, xxx good




==> doc/draft/2-related_v1.tex <==

\section{Related Work}

% We reviewed relevant literature on the empirical studies and technical systems for coding with large language models (LLM), 
% natural lanugage interfaces,
% and structural code editors.

We reviewed relevant literature on empirical studies of coding with Large Language Models (LLMs), 
human-AI collaborative systems for coding,
natural language interfaces, and structural code editors.

\subsection{Coding with LLMs}
Recent advancements in LLMs have dramatically reshaped the landscape of software development. 
These AI-driven tools,
capable of generating syntactically correct and logically sound code from natural language prompts,
have unveiled a new frontier in programming efficiency and accessibility~\cite{}.
In essence, the emergence of successful LLM-based coding tools (e.g., Github Copilot~\cite{}) marks a paradigm shift in the methodology of coding.

The interaction between programmers and LLMs has been the subject of extensive research. 
Many studies~\cite{Kazemitabaar2023,nguyen2024beginning,prather2023} have delved into understanding the nuances of this interaction, 
focusing primarily on user behavior when using LLM-based coding assistants.
% Grounded copilot: How programmers interact with code-generating models, barke2023grounded
For instance, Barke et al.~\cite{barke2023grounded}
categorized the user behavior into acceleration mode, 
where the programmer has a clear conception of the code to be written, 
and exploration mode, 
where the programmer seeks guidance or inspiration due to uncertainty about the solution.
% Reading Between the Lines: Modeling User Behavior and Costs in AI-Assisted Programming
Mozannar et al.~\cite{} proposed CUPS, a taxonomy that characterizes the 
the programmers' activities when interacting with LLMs during coding tasks.
Notably, CUPS was developed based on data labeled by the participants themselves rather
than by the researchers interpreting their actions.
% An empirical Study of developer Behaviors for Validating and Repairing Ai-Generated Code
Tang et al.~\cite{} used eye-tracking data to analyze programmers' behaviors 
and found that they had a greater cognitive effort in editing AI-generated code.

Alongside user behavior,
researchers have identified several key usability issues when coding with AI assistants.
Crafting effective prompts is a common obstacle for users~\cite{sarkar2022like}, 
necessitating a deep understanding of LLMs' interpretive mechanisms and the ability to articulate intentions clearly in natural language. 
Verifying the correctness and debugging of generated code pose difficulties, especially for those with limited programming experience~\cite{vaithilingam2022expectation}, 
potentially leading to an over-reliance on the assistant. 
Moreover, these tools often lack controllability, 
offering users minimal influence over input processing and output generation~\cite{Liang2023}. This limitation was attributed to the frequent misalignment between the model's and the programmers' attention~\cite{kou2023model}.

Building upon the rich insights from existing studies, 
our work seeks to enhance the usability of LLM-based coding tools. 
However, to achieve this objective, 
we identified a gap in the existing literature: 
an understanding of the actual prompts used by programmers in real-world settings remains elusive. 
Previous studies, such as that by Barke et al.~\cite{barke2023grounded}, 
have touched upon the distinctive nature of prompts for guiding AI compared to standard code comments, but further details remain unexplored. 
By conducting a contextual inquiry,
we aim to shed light on the
nature of programmer prompts used to guide LLMs in everyday development projects. 

\subsection{Human-AI Collaborative System for Coding}
Building on the insights laid by previous emprical studies, 
the evolution of human-AI collaborative systems for coding stands at the vanguard of addressing the usability challenges inherent in these advanced but imperfect models. 
Efforts in this domain have been geared towards fostering a more symbiotic relationship between human programmers and AI models, 
with research initiatives broadly focusing on two key objectives: 
aiding users in translating their intentions into effective prompts~\cite{yen2023coladder, angert2023spellburst, ross2023programmer, cai2023low, liu2023wants, tian2023interactive} 
and enhancing these prompts to more accurately govern the output generated by LLMs~\cite{beurer2023prompting, huang2024anpl, lahiri2022interactive}.

In the HCI community, 
there's a focus on creating interactive systems that bridge the gap between a programmer's conceptual intentions and the actual prompts. 
For instance, the Coladder~\cite{yen2023coladder} introduces a block-based user interface that enables programmers to hierarchically decompose their prompts.
This approach allows users to edit segments of their prompts, 
refining the AI-generated code in a more controlled manner.
Spellburst~\cite{angert2023spellburst} presents a node-based visual programming environment designed for creative coding.
Furthermore, the concept of Grounded Code Matching, proposed by Liu el al~\cite{liu2023wants}, shifts the paradigm from a one-way prompt-to-code process to an interactive loop. 
This method generates textual explanations alongside code, enabling users to edit these explanations and use them as refined prompts to iteratively improve the AI's output. 
Tian et al.~\cite{tian2023interactive} extended this interactive approach to SQL, showcasing its versatility across different programming domains.

In contrast, the programming languages community has explored new paradigms to transform prompts into more structured representations, thereby exerting finer control over the AI's output. Beurer-Kellner et al.~\cite{beurer2023prompting} introduced LMQL, a scripting language that blends traditional text prompts with scripts to constrain and direct the output of LLMs. 
Huang et al.~\cite{huang2024anpl} adopted a paradigm from program synthesis, utilizing ``sketches'' (i.e., control or data flow expressed in precise code) and ``holes'' (placeholders for yet-to-be-implemented parts) to guide the code generation process.
% Moreover, the concept of test-driven user-intent formalization emerged as a method to govern code generation through test cases, providing a unique blend of traditional software development practices with AI-driven coding.

Despite these advancements, implementing such systems comes with its own set of challenges. T
hese methods tend to complicate the coding process and struggle to integrate smoothly with traditional practices, such as those within Integrated Development Environments (IDEs). 
Furthermore, seamlessly combining these systems to aid in both prompt formulation and controlling model output presents an even greater challenge.
Our research aims to navigate these complexities by developing an approach that 
integrates seamlessly with the IDE,
aiding users not only in crafting their prompts 
but also in enhancing the prompts to more effectively guide the LLM's output.


% Discovering the Syntax and Strategies of Natural Language Programming with Generative Language Models
% Ai chains: Transparent and controllable human-ai interaction by chaining large language model prompts, wu2022ai

%%% maybe not that relevant
% Towards More Effective AI-Assisted Programming: A Systematic Design Exploration to Improve Visual Studio Intelli-Code’s User Experience, vaithilingam2023towards
% Stylette: Styling the web with natural language, kim2022stylette


\subsection{Natural Language Interfaces}
Natural language interfaces (NLIs) have long been the subject of study for their unique ability to let users express their intentions directly. 
Early systems, such as Put-that-there~\cite{} and Quickset~\cite{}, 
allowed users to interact with computers through verbal commands, 
marking the initial steps towards NLIs.
As natural language processing techniques evolved, 
this paradigm expanded into various domains, including data analysis~\cite{}, image editing~\cite{}, and beyond. 
However, a limitation of these systems was their requirement for users to explicitly articulate commands—even in natural language—thereby restricting the fluidity and expressiveness usually inherent in human language and its applications.

Another approach of NLIs treat users' natural language input more implicitly,
capitalizing on the latent linguistic structure within the text to foster fluid and streamlined interactions. 
For instance, CrossData~\cite{} exemplifies this approach by inferring data operations and relationships directly from textual data reports, 
thereby streamlining the process of data report authoring and reducing the need for extensive iterative interactions. 
For instance, CrossData~\cite{} exemplifies this approach by deducing data operations and relationships directly from textual data reports, thereby reducing the need for extensive iterations involved in authoring data reports, such as consistency checking, visualizations refinements, and more.
Similarly, DataParticles~\cite{} utilizes the inherent connections between text captions and graphical elements to automate the creation of animated unit visualizations.
This work follows in the footsteps of these approaches, implicitly extracting the latent linguistic structure from prompts to create code sketches on-the-fly, 
while also considering the prompt as an explicit command for LLM. 
This approach not only delivers immediate feedback to users but also affords more precise control over the outputs of LLMs.


\subsection{Structural Code Editor}
Structural code editors, different from text-based editors, 
manipulate the underlying abstract syntax tree (AST) of a program rather than its textual representation. 
This approach enables a more intuitive and error-resistant way of programming, 
as users interact with the code in more visual and structured ways.
% For example, 
% Sketch-n-Sketch~\cite{10.1145/3332165.3347925}
% % blurs the lines between making textual changes to the code and visually adjusting the graphical output, offering a more integrated experience for creating SVG graphics. 
% The use of structural editors has been embraced across various programming environments, 
% especially in educational tools and IDEs designed to simplify coding for beginners and experts alike. 
The utility and innovation of structural editors have been demonstrated through their widespread adoption and the development of numerous projects in both academic and industrial spheres~\cite{}. 

Drawing inspiration from the principles of structural editing, 
we adapt its core concepts to the task of translating natural language prompts into code. 
Instead of directly converting text to code using LLMs,
our approach leverages the latent linguistic structure of the prompt 
to edit and manipulate the structure of code via its AST. 
This method allows us to create a preliminary sketch of the code, providing immediate feedback to the user



% %% directly edit the AST instead of chars
% Structural code editors, which enable programmers to directly manipulate the high-level concepts (e.g. abstract syntax tree (AST)) rather than the textual code itself, represent a significant shift in the way code is edited and understood. 
% This approach allows for a more intuitive interaction with the underlying structure of the code, ensuring that edits are syntactically correct by design. 

% Building on this foundation, techniques such as those presented in~\cite{9127256} utilize toString functions to automatically generate graphical user interfaces (GUIs), making data structure manipulations within integrated development environments (IDEs) more accessible, particularly in programming by examples (PBE) or bidirectional transformations (BX) contexts. 

% This fusion of direct code manipulation with user interaction is further exemplified in projects like~\cite{10.1145/3332165.3347925}, which blur the lines between making textual changes to the code and visually adjusting the graphical output, thereby offering a more integrated experience for creating SVG graphics. 

% On the educational side, editors such as~\cite{10.1145/3397537.3397561} aim to make programming more approachable for beginners by ensuring that any code changes remain within the bounds of the language's syntax, thus smoothing the learning path. 
% Similarly, GNOME~\cite{10.1145/800020.808250} leverages lessons from structural editing research to create an environment conducive to learning programming, especially for novices. 

% The concerted efforts of these initiatives, along with a wide array of industrial projects~\cite{Lamdu91:online, Darklang73:online, TheUniso32:online, ensoorg70:online}, 
% underscore the continuous innovation and diverse strategies within this domain, all aimed at reconciling the intuitiveness of graphical interfaces with the precision of textual programming.

% However, while existing methods emphasize features like GUI generation, seamless graphical integration, and educational facilitation, they also highlight an area ripe for exploration: the language-oriented nature of structural code editors. This focus on tailoring editors to specific programming languages presents an opportunity to delve deeper into how these tools can adapt to diverse programming paradigms and environments. The challenge lies not in the language specificity itself but in expanding these editors' capabilities to accommodate a broader range of languages and development contexts. By exploring this area, the field can potentially address issues of adaptability and scalability, making structural code editors more universally applicable and enhancing their utility across various programming ecosystems.

% \subsection{Natural Language to Code: Model \& Algorithms}

% %% earlier stage: rule based, keyword-based snippet
% %% preLLM: ML-based
% %% LLM: werwer

% % Zeyu -- Version 2
% To enhance our understanding of the underlying principles guiding code creation by Large Language Models (LLMs), we delved into the scholarly works surrounding the models and algorithms enabling the translation of natural language into code. Initially, the field witnessed the introduction of rule-based systems, exemplified by~\citet{winograd1980does}, which demonstrated an ability to interpret natural language instructions within a simplistic block world environment. Building on these foundational concepts,~\citet{feigenbaum1980knowledge} laid the groundwork for expert systems and knowledge-based methodologies in artificial intelligence, principles that found early application in Natural Language to Code (NL2Code) systems. The subsequent phase of research shifted towards statistical methods and the nascent stages of machine learning, as illustrated by foundational works in the field~\cite{manning1999foundations, joachims1998text}.

% Advancements continued with the introduction of frameworks like GATE, which refined the approach to identifying key phrases and patterns within text~\cite{cunningham2002gate}. In more recent developments, researchers have employed structured queries to enhance the structural coherence of the generated code~\cite{beurer2023prompting, elgohary2021nl}. Parallel to this, the concept of flow engineering has been employed to maintain the structural integrity within code generation~\cite{ridnik2024code, reynolds2021prompt}. The application of Abstract Syntax Trees (AST) represents another significant stride, facilitating the parsing of generated code and linking code structures with natural language elements~\cite{yin2018tranx, 10.1145/3611643.3616323}. These approaches collectively highlight the intricate interplay between grammatical rules and semantic understanding in code generation, marrying deterministic frameworks with the creative aspects of code production.

% However, the integration of rule-based precision with the creative freedom of generative models remains a formidable challenge. Addressing this, Yin et al. introduced a groundbreaking neural framework that integrates a grammatical model to embed prior syntactic knowledge, aiming to harmonize the rigor of rule-based systems with the adaptability of generative models. This equilibrium is pivotal for bolstering the efficiency and dependability of code generated by LLMs~\cite{yin2017syntactic}.


==> doc/draft/3-formative_study.tex <==

\section{Understanding Code References in Prompts}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{figs/code_reference.pdf}
    \caption{Code Reference.}
    \label{fig:code_reference}
\end{figure}

The goal of this work is to investigate the utilization of linguistic structures inherent in prompts for transforming them into code sketches. 
Central to this language-oriented approach is identifying the correspondences between phrases within the prompt and elements of the code. 
We refer a word or phrase within a prompt as a \emph{Code Reference}
if it specifically points to a piece of code (formally a node on the Abstract Syntax Tree~\cite{}).
These phrase-level references serve as anchor points, linking the prompt's linguistic structure to specific code elements, and play a crucial role to achieve our goal since we aim to update the code sketch incrementally as the user types.
\zt{why? should justify more}

To inform our approach, we conducted a contextual inquire aimed at understanding the reasons, 
methods, 
and contexts in which users employ code references in their prompts. 

\subsection{Study Setup}
% - participants
% - procedure
% - analysis

\paragraph{Participants.}
We recruited 11 participants through university mailing lists and forums, selecting them based on a screening questionnaire that assessed programming proficiency and experience with AI Coding Assistants (e.g., GitHub Copilot or ChatGPT). 
Our focus was on individuals who utilized textual prompts to guide AI models in coding tasks, 
excluding those who solely relied on the auto-complete feature of these models. 
Participants were required to present a recent project where they employed LLMs for coding. 
Participant backgrounds are detailed in Table~\ref{table: formative participants}.

\begin{table}[!tbh]
\resizebox{\linewidth}{!}{
\begin{tabular}{cccl}
\toprule
    & \textbf{Years on Coding} & \textbf{Frequency of using LLMs} & \textbf{Project Type}                    \\ \midrule
P1  & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P2  & 5+                            & Daily                        & Front-end Development          \\ \hline
P3  & 5+                            & Always                       & Front-end Development          \\ \hline
P4  & 5+                            & Always                       & Machine Learning                    \\ \hline
P5  & 5+                            & Monthly                      & Back-end Development           \\ \hline
P6  & 3-5                           & Daily                           & Back-end Development            \\ \hline
P7  & 3-5                           &  Always                       & Machine Learning                    \\ \hline
P8  & 5+                            &  Always                        &  Front-end Development        \\ \hline
P9  & 5+                              &  Daily                            &  Front-end Development      \\ \hline
P10 & 3-5                           & Weekly                       & Data Analysis \& Visualization \\ \hline
P11 & 1-2                           &  Weekly                            & Embedded Systems Development    \\ \hline
\end{tabular}
}

\caption{Participants in Formative Study}
\label{table: formative participants}
\end{table}

\paragraph{Procedure.}
Our study is designed to understand how participants interact with LLMs within their coding workflows. 
The study is structured into a warm-up session (5mins), a contextual inquiry(30mins), and a final interview (20mins).
In the warm-up phase, participants open their IDE and share a recent experience using LLMs for code generation beyond simple code completion. 
Following the warm-up is a contextual inquiry.
Participants work on an ongoing project, using LLMs while verbalizing their thought process. 
We note observations for further exploration in the interview phase.
The study concludes with an interview, 
diving into the experiences and perceptions highlighted during the inquiry. 
We also discuss their overall experience with LLMs to gather comprehensive feedback. 
This interview is conducted via Zoom and recorded (both video and audio) for analysis.
Participants provided consent and were compensated with \$20 for the 60-minute session.

\paragraph{Data Analysis.}
The interviews were audio-recorded, transcribed, and independently coded by three co-authors. Discrepancies in coding were resolved through discussion. 
Additionally, we collected and examined the prompts used by participants, as well as the corresponding code generated during the contextual inquiry, using the video recordings to deepen our understanding of the exact text used by the participants and its context.
Our analysis employed the thematic analysis method, generating the codes and themes both 
 both inductively (i.e., bottom-up) and deductively (i.e., topdown),
The final themes were established after three rounds of iterative refinement.

\subsection{Findings \zt{WIP}}

% \subsubsection{Coding with LLMs in The Wild: Scenarios \& Behaviors}

% We observed distinct categorizations and behaviors among users engaging with coding assistant tools, specifically focusing on their tasks and coding expertise. 
% Our contextual inquiry revealed a dichotomy in user needs based on their coding skills: experienced programmers (N = 5) often rely on automated code completion features to enhance productivity without overwhelming their codebase, valuing control and clarity in their coding process. 
% Conversely, novices or those new to specific coding tasks (N = 6) showed a preference for using interactive chat features to navigate and understand coding practices more exploratively. 
% When considering the nature of coding tasks, front-end developers emphasized code quality, prioritizing well-structured components, and refactoring, while algorithm developers concentrated on optimizing logic and efficiency, posing a challenge for the coding assistant's comprehension due to the abstract nature of these requirements. 
% Feature usage patterns also emerged, with users employing strategies such as adding function inputs/outputs to prompts and enhancing function parameters for clearer guidance. 
% Additionally, integrating web context into the coding assistant's workflow emerged as a valuable approach, where users first seek insights online before consulting the coding assistant, thereby enriching the context and improving the relevance of the assistant's suggestions.

\subsubsection{Reasons of Using Code References}

% Referring code elements using phrases is a common behavior in our participants (\zt{data}).
% Per our observation, there are primary three reasons of referring code elements in the prompts.
% First, in most of the cases, participants use code references with the intent to better control the code generations.
% Second, participants use code reference due to their expressiveness, which, server as a symbolic references that capture the context of the code, such as its type, environment, and relationships to other codes. Sometimes it would be difficult to compose the prompt without refering to a code element.
% Finally, participants use code reference in their prompt due to the inherent limited of textual representation.
% They don't have other modality to refer code elements in their prompt. this is examplify by using the feature of inline chat, where the participants can select a piece of code and then comment on it.

Referring to code elements through phrases is a common practice among our participants, driven by three primary reasons. 
Firstly, participants often employed code references to enhance control of LLM over the code generation process.
Secondly, participants used code references due to their expressiveness. These references act as symbolic markers that encapsulate the code's context, including its type, environment, and interrelations with other code segments.
As a result, sometimes it challenging to formulate prompts without such references. 

Lastly, the reliance on code references is partly attributed to the limitations of textual representation in prompts. Given the absence of alternative modalities to indicate code elements, participants frequently utilize features like inline chat to highlight specific code pieces and provide contextual commentary. This practice underscores the necessity of code references in bridging the communicative gap between the participants' intent and the LLM's understanding.


% A significant hurdle in mastering controllability lies in the inherent difficulty of specifying the scope and extent of desired changes. The current mechanisms of auto-completion and inline chat offer limited avenues for users to convey comprehensive information and context to the model, thereby constraining their ability to direct its output accurately. Specifically, LLMs cannot provide instant feedback, like \textit{P10} said: ``If I could know what to change in the specific corresponding code while writing the prompt (in real-time), it would be useful in debug or learning code scenarios.''. This challenge is further exacerbated for users who may not possess the eloquence or experience to articulate their requirements effectively. Moreover, the pursuit of controllability transcends simple prompt adjustments, highlighting a complex interaction between the prompt's content and the broader context that is situated. Ideally, controllability should emerge from a harmonious blend of both of these elements. However, the absence of instant feedback mechanisms introduces a layer of opacity to the model's operational logic, leaving users to navigate a series of "black box" processes. This lack of transparency significantly impedes the user's capacity to influence the model's behavior in a predictable and desired manner.

% As we culminate our findings, it's crucial to acknowledge that the challenges in achieving controllability may stem, in part, from the stochastic nature of LLMs themselves. The probabilistic and often unpredictable outputs generated by these models necessitate a more structured approach to prompting. To mitigate the inherent unpredictability and enhance user control, there's a pressing need for the development of structured rules and frameworks that can guide users in crafting their prompts. Such guidelines would not only facilitate more precise interactions with LLMs but also potentially alleviate the cognitive load on users, allowing them to delegate some of the model's tasks more effectively and efficiently. This shift towards a more rule-based prompting strategy underscores the ongoing evolution in our understanding and utilization of LLMs, particularly in the realm of coding and software development.


\subsubsection{Types of Code References: Independent and Dependent}

In analyzing how participants refer to code in their prompts, 
we identify two types of references: \emph{independent} and \emph{dependent}.

\begin{itemize}[leftmargin=*]
    \item \emph{Independent Reference} standalone points to code elements, typically employing the exact identifier of these elements (e.g., variable or function names) or reserved keywords. 
    The code referent of an independent reference can be precisely located without extra contextual information in the prompt. 
    For example, \zt{example} \textcolor{red}{(1) Converts $t_x$ and $t_y$ to pixel-based coordinates, (2) print the shape of $SalePrice$ in train.csv, (3) start reading data when you see \$ sign, stop reading data when you see \# sign, etc.}
    % when a participant uses "Initialize array dataStorage", "array" acts as an independent reference. The term directly points to a specific code construct, and dataStorage identifies the exact variable involved, allowing for clear and immediate identification within the codebase.
     \textcolor{red}{Edit code \textbf{above}; Add \textbf{this}, with model save name automated; the return type of \textbf{this} function is a node list }
     \textcolor{red}{\textbf{write} data to the serial port; \textbf{Convert} the string data to floating-point numbers}

    \item \emph{Dependent Reference}, on the other hand, refers to code elements through their relationship with other references within the prompt.
    The code referent of a dependent reference cannot be accurately located without additional information provided by the surrounding text.
    For example, \zt{example}
    % The referent of "it" (i.e., the array dataStorage) is understood only by considering its relationship with the independent reference that precedes it.
\end{itemize}

Identifying how a reference refer to code helps in developing strategies for parsing prompts as the user types and mapping them to code elements.

\subsubsection{Context of Code References: An Intermediate Level of Clarity}
In our study, we found that users often refer to code elements when they possess an intermediate level of clarity about the desired code.
Previous research~\cite{} has categorized user interactions with LLM-based programming assistants into two modes: acceleration, characterized by a clear vision of the intended code, and exploration, marked by uncertainty about the solution. 
Our observations echo these distinctions, 
revealing that users in exploration mode often 
describe their problems rather than specify code elements, 
utilizing tools like ChatGPT or Copilot Chat for guidance. 
Conversely, those in acceleration mode lean towards direct code manipulation, 
favoring features like Copilot's auto-completion instead of NL prompts.

In addition to exploration and acceleration mode,
we also noticed that participants often have an intermediate clarity of the intended code -- a state where the user possesses an overall conceptions of the necessary functions, variables, or code structures but lacks confidence in the finer details.  
For instance, a user might request the creation of a \emph{``REST API with a GET handler to read from a database''}, 
implying a clear idea of the desired code element (i.e., \emph{a GET handler}) 
reveals ambiguity about how to achieve this functionality (i.e., how to \emph{read from a database}).
This intermediary position encourages more frequent referencing of code elements as users seek to align the generated code with their project's architectural goals and details.
In this intermediate clarity zone, 
participants find Copilot Inline Chat or inline comments to be more suitable.

It's crucial to acknowledge that our classification of user behavior represents a spectrum rather than discrete categories. Users dynamically transition among these states throughout the coding process, reflecting the fluid and dynamic nature of software development.
These observations not only highlight the versatility required of LLM-based programming assistants 
but also pinpoint the specific scenario where our Language-Oriented Code Sketching approach can offer the most value.



% \subsubsection{Prompts: Abstraction Levels}
%Transitioning to the medium abstraction level, we observed a more intricate interplay between the user's intention and the inclusion of specific details. This is exemplified by prompts from participants like: ``Color scale based on ‘cluster’ column, 10 colors'' -- \textit{P10}, ``Plot the correlation between the top 10 features with highest correlation using a heat map, only showing top 10'' -- \textit{P1}. These prompts skillfully combine the what and the how, guiding the assistant while preserving the user's strategic goals. Conversely, some participants adopts an alternate medium-level strategy by outlining the technical specifics before revealing the broader objective, as seen in their prompt to ``Add parameters x / y to the function so that I can manage them'' -- \textit{P5}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% F1 - observation: 
%     - abstraction level
%         - prompt scope
%     - prompt is a combination of text and code: 

%     F?
%     - contextual inquire -- using copilot in the wild: a large portion of code / entire project. Key takeaways?

%     - middle level - fuzzy + concrete, need an example to explain
%     - lack of code-prompt pairs
%     - lack of history
    
%  -- why / when to write prompt (fix errors, add input / output)
    
% F2 - pain points
%    - Lack of Instant Feedback (Slow feedback) / Controllability
%     - learning by error and trial - need iterations
    
%    - Huge code generated, regenerate from sketch, mess up
%    - Intensive Work of code + prompt combination
%     - scope control --> 
    
% F3 - Design Implication


% \subsubsection{Iterations: Learning by Trial and Error}

% Building on our examination of how users navigate the abstraction levels in their prompts, our investigation extends into the iteration phase, which unveils the intricate dynamics of user engagement with coding assistants. We observed a significant investment of time and effort by participants, particularly when engaging in the iterative process of refining both prompts and the generated code. This process was notably pronounced at the middle and low levels of abstraction, where the balance between controlling the output and efficiently achieving desired results becomes a delicate dance. 

% The quest for control over the coding assistant's output through prompt adjustments emerged as a formidable challenge, more so when users are faced with lengthy and complex code segments. This aspect of interaction becomes exceedingly strenuous at lower abstraction levels, where the precision in prompt crafting demands a substantial investment of time and cognitive effort. When the generated code deviates from the expected outcome, users find themselves ensnared in a time-consuming cycle of trial and error, attempting to refine prompts with the hope of steering the code generation closer to their desired intent. However, our observations indicate a pragmatic threshold among many participants (N=7), who exhibited a reluctance to exceed an average of 2 to 3 iterations of prompt modification. Beyond this point, the inclination shifts towards engaging directly with the code itself, opting for manual modifications over further prompt refinements. This transition from relying on the coding assistant's capabilities to applying personal coding acumen highlights a critical juncture in the iterative development process, illuminating the balance users strike between the convenience of automated assistance and the autonomy of hands-on code manipulation.







\subsection{Conclusion}

\newpage
% Our exploration into the interaction between users and large language models (LLMs) in coding contexts reveals a complex landscape marked by diverse user needs, the nuanced use of prompts, iterative refinement processes, and significant challenges in controllability. We observed a broad spectrum of user behaviors, from experienced programmers prioritizing control over their code to novices exploring coding concepts through interactive chats. The categorization of prompts into varying levels of abstraction highlighted the delicate balance users strive to achieve between specificity and generality, often leading to a labor-intensive cycle of trial and error as they seek to refine both prompts and the resulting code. This iterative process, while fostering a deeper understanding of the code, often culminates in a feeling of tedium and a lack of control, exacerbated by the stochastic nature of LLM outputs and the absence of instant feedback mechanisms. \textbf{These insights underscore the need for a transformative approach to LLM-assisted coding, one that integrates instant feedback and incremental prompt and code updates within a structured, interactive system.} By addressing these core issues, we can enhance the efficiency, controllability, and overall user experience of coding with LLMs, paving the way for more intuitive and empowering developer tools.

==> doc/draft/4-method_v1.tex <==


\section{\method{}}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\columnwidth]{figs/interaction_loop.pdf}
    \caption{Interaction Loop.}
    \label{fig:inter_loop}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{figs/ui_exp.pdf}
    \caption{UI Example.}
    \label{fig:ui_exp}
\end{figure}

% \begin{figure*}[bh]
%     \centering
%     \includegraphics[width=2\columnwidth]{figs/pipeline_exp.pdf}
%     \caption{Method Pipeline.}
%     \label{fig:pipeline_exp}
% \end{figure*}

% Selecting a completion previews its integration into the existing code in the code editor , 
% and if accepted, the snippet is inserted.
% Upon selecting a completion, 
% the system previews where the code snippet will be inserted into the existing code (\autoref{fig:ui_exp}\cmo{a}).
% Should the user accept the completion, the code snippet is inserted. 


\noindent
We seek to create an intermediate result during the prompt-typing process, 
which accomplishes two key goals: 
1) offering users instant, incremental feedback, 
and 2) serving as a base to guide the LLM's code generation. 
To this end, we design \textbf{\method{}}, 
an interactive approach that that instantly and incrementally transforms a user's prompt into a code sketch.

Our approach leverages \emph{``word completion''} as an interface to incrementally construct the code sketch, 
fostering a seamless collaboration between human and machine intelligence.
\autoref{fig:inter_loop} shows the interaction loop between a user and the system,
encompassing three key steps:
\begin{enumerate}
    \item \textbf{Map and Suggest}.
    As a user types the prompt, 
    the system maps the current typing phrase to a list of potential corresponding code elements,
    and suggests completions for the phrase based on the code elements (\autoref{fig:ui_exp}\cmo{b}). 

    \item \textbf{Assemble and Preview}.
    When the user selects a completion,
    the system integrates its corresponding code elements with the existing code
    and provide a preview of the result (\autoref{fig:ui_exp}\cmo{a}).

    \item \textbf{Insert and Preserve}.
    Once the user accepts the completion, the system inserts the completion to the prompt and its corresponding code elements to the code editor.
    The system then preserves the connection between the prompt phrase and the corresponding code elements.
\end{enumerate}

The user can submit their prompt and the code snippet to LLMs at any preferred moment.
Next we explain the detail of the three key steps.

\subsection{Map and Suggest}
When a user types a word,
we aim to dynamically map this word to the corresponding code element,
whether it exists in the code editor or not.
Due to the ambiguity in natural language, 
we decide to derive multiple potential mappings as suggestions
rather than a single definitive result. 
Based on our analysis in Sec.~\ref{sec:code_ref},
a word can either be an independent or dependent code reference.
Thus, we use different strategies to suggest code elements:


\subsubsection{\textbf{Matching Predefined Code Snippets or Existing Code}}
    If a word is an independent code reference,
    it can standalone refer to a code element.
    Thus, we use a fuzzy string matching to match the word with
    two sources of code elements (\autoref{fig:ui_exp}\cmo{X}):

    \begin{itemize}
        \item \emph{Predefined Code Snippets.} 
        % We match the typed word with predefined code snippets.
        We provide a list of code snippets as potential matches for the typed word. 
        A code snippet is a small block of re-usable code, ranging from simple code fragments to complex function or class templates.
        Modern IDEs often provide predefined snippets.
        For example, there are more than 7 thousand snippet extensions for VS Code.

        \item \emph{Existing Code.}
        We also dynamically parses the existing code to suggest \emph{identifiers}, such as function names or variables, as potential matches for the typed word.       
    \end{itemize}
    
\subsubsection{\textbf{Inferring Based on Linguistic Features}}

If a word is a dependent code reference,
we need to use the linguistic context to infer the code elements it refers to.
We use two NLP techniques to infer the corresponding code elements:

    \begin{itemize}
        \item \emph{Part-of-Speech.}
        In user's prompt, nouns usually indicate variables, while verbs suggest functions~\cite{}.
        Recognizing these patterns, 
        we employ a \emph{part-of-speech tagging} of the word and map it to a variable or function accordingly.
        For example, \autoref{fig:pipeline_exp}\cmo{X} shows that the system maps the word ``layer'' to attributes in the class, while xxx function.
        
        % allows us to map each word to the most appropriate code element based on its part of speech. This insight helps us tailor our suggestions to align with the user’s coding intentions.
        % In user prompts, nouns often signify variables, while verbs typically suggest functions or actions. 
        \item \emph{Co-reference.}
        Certain phrases, such as ``it'' or ``the function'', commonly refer back to other specific phrases mentioned earlier in the user's prompt. 
        Through co-reference analysis, we can map these phrases to the corresponding code elements of the earlier 
        phrases they refer to.
        
    \end{itemize}

% A critical challenge of our approach is efficiently and meaningfully mapping typed words to potential code snippets for immediate feedback. 
% Our approach draws upon three sources to suggest corresponding code snippets:

% \para{Step1. Mapping the Word to Potential Code Snippets.}
% \para{Step1. Completing the word being typed.}
% % Word completion is a staple in modern text editors, 
% % designed to streamline typing~\cite{}. 
% % Our implementation employs a predefined dictionary and fuzzy string matching to suggest completions for the word being typed.
% % We leave enhancement with more sophisticated methods for the future.
% Word completion, a common feature in modern text editors, enhances typing efficiency~\cite{}. 
% Our system utilizes a predefined dictionary and fuzzy string matching to offer word completion suggestions, 
% aiming to incorporate more advanced techniques in future enhancements.
% \zt{informed by the formative study: Independent reference and dependent reference}


\subsection{Assemble and Preview}
After mapping a phrase to a potential code element,
the next key challenge involves assembling it with other existing code elements.
Our observation is that the prompt often incompass rich linguistic structures that indicate the relationships between the code elements.
For example, \zt{an example.}
Based on this observation, we try to leverage the linguistic structures to generate assemblings and preview the results for the user in the code editor.
% the suggested code snippet into the existing code 
% and previewing it for the user.

Specifically, given the current word and its corresponding code element,
our approach involves two steps to assamble it with previous code elements:
\begin{enumerate}
    \item Dep parsing, which get us a tree
    To achieve this, we first employ a dependency parsing~\cite{} to obtain the
linguistic relationships between the current word and other code-associated words.

    \item recursively verify the relationship between the current word and its parents who is code references. if their relationship matches rules in a predefine rulessets, try to assemble it.
    The assemble process also consider the PL grammars.
    Subsequently, we examine the pairwise relationships between the typed word and each code-associated word. 
When a relationship matches our predefined rules \cmo{examples?},
our system recommends an insertion point within the code's AST, 
considering the code's grammatical aspects such as types and syntax.

\end{enumerate}


\autoref{fig:pipeline_exp} shows an example, where the user is typing ``laye''.
Our system auto-completes this to ``layer'' (Step1) and 
identifies it as a noun, thus mapping it as a variable (Step2).
Through dependency parsing (\autoref{fig:pipeline_exp}a), 
our system recognizes ``layer'' as an object of a preposition of the  
``PyTorch module'' (\autoref{fig:pipeline_exp}b), 
which is associated with a class definition.
Consequently, we propose adding ``layer'' as a new child node in the class's AST (\autoref{fig:pipeline_exp}c), 
thereafter rendering this suggestion as code and providing a preview within the code editor for user validation.

\subsection{Insert and Preserve}

\para{Step3. Maintaining Word-Code Associations.}
Once a user accepts a suggested insertion, 
our system maintains the established association between the word and its corresponding code. 
This preserved relationship is crucial for the system to support incrementally building the code sketch. 
As the user inputs additional words, our system utilizes these prior associations to propose potential insertion points for new code (Step 3). 

\subsection{Discussion}

\subsection{The applicability of \method{}}

\para{AST rate.}

\para{Failure Cases}

- how robust is our method
- failure cases


==> doc/draft/6-user_study.tex <==
\section{User Study}

To assess the usability and performance of our prototype, a comparative user study was conducted, juxtaposing our system with the Copilot inline chat.

\subsection{Study Setup}

\paragraph{Participants}
We enlisted \textcolor{red}{16} participants with an average age of \textcolor{red}{23.6}, who were proficient in programming and experienced in using large language models (LLMs). Selection was based on a screening questionnaire that evaluated their programming skills and familiarity with LLMs.

\paragraph{Procedure}
The whole study lasted for around 60-70 minutes. Participants could partake in the study either remotely or in person. Initially, we allocated five minutes for setting up the environment for each participant. For those joining remotely, our prototype was hosted on a publicly accessible online server. In contrast, in-person participants accessed it through localhost. This was followed by a 15-minute tutorial session, designed to acquaint participants with our system. Subsequently, they were tasked with completing two specific assignments (each task time limited to 15 minutes): Task 1 involved implementing a Python Flask server, and Task 2 focused on developing a Pytorch module for machine learning. To mitigate learning effects and introduce variability in the study, a counterbalanced method was employed. This approach involved having half of the participants commence with Task 1 using our prototype and Task 2 with the baseline system, and the order was reversed for the rest. For each task, participants were required to complete three rounds. In each round, they were given pseudo code to serve as a reference. This pseudo code included multiple checkpoints, which were used to evaluate and score the participants' performance. Participants were encouraged to utilize the instant feedback feature extensively. However, they were also permitted to submit prompts to GPT or directly modify the code within the code editor. In the baseline condition, participants used our interface to enter their prompts and interact with LLMs. However, unlike our system, they did not receive real-time feedback or incremental code updates as they typed their prompts. Finally, the participants were asked to fill in a post-study questionnaire and take a brief interview in 5-10 minutes.

\paragraph{Data Analysis}
For data analysis, we meticulously recorded the task completion time for each round, along with the pass rate, which was determined based on whether all checkpoints were met. Additionally, we evaluated the post-study questionnaire responses from each participant, which covered aspects such as controllability and accuracy of code generation, understanding of the code, efficiency, productivity, ease of use, learning curve, satisfaction and preference, system usability, and cognitive load. These aspects were rated using a 7-point Likert scale.


%% Comparitive study:
%% Copilot Inline Chat vs Ours

%% introduction task

%% 3 study Tasks:
%% difficulties lv
%% http server, the server should listent at \login for POST request.

%% time
%% sucessful rate
%% num of iterations ? prompt changes?
%% qualitative feedback

\subsection{Results}

%% post-study questionnaire

%%% 
